Thermodynamic formalism for subsystems of expanding Thurston maps II

Expanding Thurston maps were introduced by M. Bonk and D. Meyer with motivation from complex dynamics and Cannon's conjecture from geometric group theory via Sullivan's dictionary. In this paper, we study subsystems of expanding Thurston maps motivated via Sullivan's dictionary as analogs of some subgroups of Kleinian groups. We prove the uniqueness and various ergodic properties of the equilibrium states for strongly primitive subsystems and real-valued H\"older continuous potentials, and establish the equidistribution of preimages of subsystems with respect to the equilibrium states. Here, the sphere $S^{2}$ is equipped with a natural metric, called a visual metric, introduced by M. Bonk and D. Meyer. As a result, for strongly primitive subsystems of expanding Thurston maps without periodic critical points, we obtain a level-$2$ large deviation principle for Birkhoff averages and iterated preimages.

==> section/Asymptotic_expansiveness.tex <==
% !TEX root = ../main.tex

\section{Asymptotic \texorpdfstring{$h$}{h}-expansiveness}
\label{sec:Asymptotic h-expansiveness}

% In this section we study weak expansion properties for subsystems of expanding Thurston maps.

\subsection{Basic concepts}%
\label{sub:sec:Asymptotic h-expansiveness:Basic concepts}

We first introduce some terminology and definitions.

Let $X$ be a compact metrizable topological space and $g \colon X \mapping X$ a continuous map. 

A \defn{cover} of $X$ is a collection $\xi = \{ A_j \describe j \in J \}$ of subsets of $X$ with the property that $\bigcup \xi = X$, where $J$ is an index set. 
The cover $\xi$ is an \defn{open cover} if $A_j$ is an open set for each $j \in J$. 
The cover $\xi$ is \defn{finite} if the index set $J$ is a finite set.

Let $\xi = \{ A_j \describe j \in J \}$ and $ \eta = \{ B_k \describe k \in K \}$ be two covers of $X$. 
We say that $\xi$ is a \defn{refinement} of $\eta$ if for each $A_j \in \xi$, there exists $B_k \in \eta$ such that $A_j \subseteq B_k$. 
For two covers $\xi$ and $\eta$, the \defn{common refinement} $\xi \vee \eta$ of $\xi$ and $\eta$ defined as
\[
	\xi \vee \eta \define \{ A_j \cap B_k \describe j \in J, \, k \in K \},
\]
which is also a cover of $X$. 
Note that if $\xi$ and $\eta$ are both open covers, then $\xi \vee \eta$ is also an open cover. 
Define $g^{-1}(\xi) \define \{ g^{-1}(A_j) \describe j \in J \}$, and denote for $n \in \n$,
\[
	\xi^n_g \define \bigvee\limits_{j = 0}^{n - 1} g^{-j}(\xi) = \xi \vee g^{-1}(\xi) \vee \cdots \vee g^{-(n - 1)}(\xi).
\]

\begin{definition}[Refining sequences of open covers]    \label{def:refining sequences of open covers}
	A sequence of open covers $\{ \xi_i \}_{i \in \n_0}$ of a compact metric space $X$ is a \defn{refining sequence of open covers} of $X$ if the following conditions are satisfied
	\begin{enumerate}
		\smallskip
		\item     \label{item:def:refining sequences of open covers:refining}
		$\xi_{i + 1}$ is a refinement of $\xi_i$ for each $i \in \n_0$.

		\smallskip

		\item     \label{item:def:refining sequences of open covers:generator}
		For each open cover $\eta$ of $X$, there exists $j \in \n$ such that for each $i \geqslant j$, $\xi_i$ is a refinement of $\eta$.
	\end{enumerate} 
\end{definition}

The topological tail entropy was first introduced by M.~Misiurewicz under the name ``topological conditional entropy'' \cite{misiurewicz1973diffeomorphism, misiurewicz1976topological}. 
Here we adopt the terminology in \cite{downarowicz2011entropy} (see \cite[Remark~6.3.18]{downarowicz2011entropy}).

\begin{definition}[Topological conditional entropy and topological tail entropy]    \label{def:topological conditional and tail entropy}
	Let $X$ be a compact metrizable topological space and $g \colon X \mapping X$ a continuous map. 
	The \defn{topological conditional entropy} $h(g|\lambda)$ of $g$ given $\lambda$, for some open cover $\lambda$, is defined as
	\begin{equation}    \label{eq:def:topological conditional entropy}
		h(g|\lambda) \define \lim\limits_{\ell \to +\infty} \lim\limits_{n \to +\infty} \frac{1}{n} H \parentheses[\bigg]{ \bigvee\limits_{i = 0}^{n - 1} g^{-i}(\xi_{\ell}) \bigg| \bigvee\limits_{j = 0}^{n - 1} g^{-j}(\lambda) },
	\end{equation}
	where $\{\xi_{\ell}\}_{\ell \in \n_0}$ is an arbitrary refining sequence of open covers, and for each pair of open covers $\xi$ and $\eta$,
	\begin{equation} \label{eq:def:relative cardinality entropy}
		H(\xi | \eta) \define \log \parentheses[\Big]{ \max_{A \in \eta} \set[\big]{ \min \set[\big]{\card{\xi_A} \describe \xi_A \subseteq \xi, \, A \subseteq \bigcup \xi_A } } }
	\end{equation}
	is the logarithm of the minimal number of sets from $\xi$ sufficient to cover any set in $\eta$. 

	The \defn{topological tail entropy} $\tailentropy{g}$ of $g$ is defined by
	\begin{equation}   \label{eq:def:topological tail entropy}
		\tailentropy{g} \define \lim\limits_{m \to +\infty}  \lim\limits_{\ell \to +\infty} \lim\limits_{n \to +\infty}  \frac{1}{n} H 
		\parentheses[\bigg]{ \bigvee\limits_{i = 0}^{n - 1} g^{-i}(\xi_{\ell}) \bigg| \bigvee\limits_{j = 0}^{n - 1} g^{-j}(\eta_m) } ,
	\end{equation} 
	where $\{\xi_{\ell}\}_{\ell \in \n_0}$ and $\{\eta_m\}_{m \in \n_0}$ are two arbitrary refining sequences of open covers, and $H$ is as defined in \eqref{eq:def:relative cardinality entropy}.
\end{definition}

The limits in \eqref{eq:def:topological conditional entropy} and \eqref{eq:def:information function} always exist, and both $h(g|\lambda)$ and $\tailentropy{g}$ are independent of the choices of refining sequences of open covers $\{\xi_{\ell}\}_{\ell \in \n_0}$ and $\{\eta_m\}_{m \in \n_0}$, see \cite[Section~6.3]{downarowicz2011entropy}, especially the comments after \cite[Definition~6.3.14]{downarowicz2011entropy}.

The topological tail entropy $h^*$ is also well-behaved under iterations, as it satisfies 
\begin{equation}   \label{eq:topological tail entropy under iterations}
	\tailentropy{g^{n}} = n \tailentropy{g}
\end{equation}
for each $n \in \n$ and each continuous map $g \colon X \mapping X$ on a compact metric space $X$ (\cite[Proposition~3.1]{misiurewicz1976topological}).

\begin{remark}    \label{rem:relation between topological entropy and tail entropy and refinement decrease tail entropy}
	The topological entropy of $g$ (see Subsection~\ref{sub:thermodynamic formalism}) is $\topoentropy{g} = h(g|\{X\})$, where $\{X\}$ is the open cover of $X$ consisting of only one open set $X$ (see for example, \cite[Section~6.1]{downarowicz2011entropy}). 
	It is also clear from Definition~\ref{def:topological conditional and tail entropy} that for open covers $\xi$ and $\eta$ of $X$, we have $h(g|\xi) \leqslant h(g|\eta)$ if $\xi$ is a refinement of $\eta$.
\end{remark}

The concept of $h$-expansiveness was introduced by R.~Bowen in \cite{bowen1972equidistribution}. We adopt the formulation in \cite{misiurewicz1976topological} (see also \cite{downarowicz2011entropy}). 

\begin{definition}[$h$-expansiveness]    \label{defHExp}
A continuous map $g\: X\rightarrow X$ on a compact metric space $X$ is called \defn{$h$-expansive} if there exists a finite open cover $\lambda$ of $X$ such that $h(g|\lambda)=0$.
\end{definition}


A weaker property was then introduced by M.~Misiurewicz in \cite{misiurewicz1973diffeomorphism} (see also \cite{misiurewicz1976topological, downarowicz2011entropy}).

\begin{definition}[Asymptotic $h$-expansiveness]    \label{def:asymptotic h-expansiveness}
	We say that a continuous map $g\colon X \mapping X$ on a compact metric space $X$ is \defn{asymptotically $h$-expansive} if $\tailentropy{g} = 0$.
\end{definition}







\subsection{Technical lemmas}  \label{subsctWeakExpLemmas}

Now we go back to the dynamical system $(S^2,f)$ where $f$ is an expanding Thurston map.


We need the following four lemmas for the proof of the asymptotic $h$-expansiveness of expanding Thurston maps with no periodic critical points.

\begin{lemma}[Uniform local injectivity away from the critical points]   \label{lmLocInjectAwayFromCrit}
	Let $f$, $d$ satisfies the Assumptions. Then there exists a number $\delta_0 \in (0,1]$ and a function $\tau\: (0,\delta_0]\rightarrow (0,+\infty)$ with the following properties:
	\begin{enumerate}
		\smallskip
		\item[(i)] $\lim\limits_{\delta \to 0} \tau(\delta) = 0$.

		\smallskip
		\item[(ii)] For each $\delta \leq \delta_0$, the map $f$ restricted to any open ball of radius $\delta$ centered outside the $\tau(\delta)$-neighborhood of $\crit f$ is injective, i.e., $f|_{B_d(x,\delta)}$ is injective for each $x \in S^2 \setminus N_d^{\tau(\delta)}(\crit f)$.
	\end{enumerate}
\end{lemma}

==> section/Co-homologous.tex <==
% !TEX root = ../main.tex

\section{Equidistribution}
\label{sec:Equidistribution}

In this section, we show in Theorem~\ref{thm:subsystem exact with respect to equilibrium state} that if $f$, $\mathcal{C}$, $d$, and $\potential$ satisfied the Assumptions in Section~\ref{sec:The Assumptions}, and $F \in \subsystem$ is strongly primitive, then the measure-preserving transformation $\limitmap$ of the probability space $(\limitset, \equstate)$ is exact (Definition~\ref{def:exact}), and as an immediate consequence, mixing (Corollary~\ref{coro:subsystem mixing}). 
Another consequence of Theorem~\ref{thm:subsystem exact with respect to equilibrium state} is that $\equstate$ is non-atomic (Corollary~\ref{coro:subsystem equilibrium state non-atomic}).

\smallskip


In this section, we will discuss equidistribution results for preimages. Let $f$, $d$, $\phi$, $\alpha$ satisfy the Assumptions and let $\mu_\phi$ be the unique equilibrium state for $f$ and $\phi$ throughout this section. We prove in Proposition~\ref{propWeakConvPreImgWithWeight} three versions of equidistribution of preimages under $f^n$ as $n\longrightarrow +\infty$ with respect to $\mu_\phi$ and $m_\phi$ as defined in Corollary~\ref{corMandMuUnique}, respectively. Proposition~\ref{propWeakConvPreImgWithWeight} partially generalizes Theorem~1.2 in \cite{Li13}, where we established the equidistribution of preimages with respect to the measure of maximal entropy. In Theorem~\ref{thmASConvToES}, we generalizes Theorem~7.1 in \cite{Li13} following the idea of J.~Hawkins and M.~Taylor \cite{HT03}, to show that for each $p\in S^2$, the equilibrium state $\mu_\phi$ is almost surely the limit of 
\[
    \frac{1}{n}\sum\limits_{i=0}^{n-1} \delta_{q_i}
\]
as $n\longrightarrow +\infty$ in the weak$^*$ topology, where $q_0 = p$, and for each $i\in\N_0$, the point $q_{i+1}$ is one of the points $x$ in $f^{-1}(q_i)$, chosen with probability proportional to $\deg_f(x) \myexp{\widetilde\phi(x)}$, where $\widetilde\phi$ is defined in (\ref{eqDefPhiTilde}).




\begin{prop}  \label{propWeakConvPreImgWithWeight}
Let $f$, $d$, $\phi$, $\alpha$ satisfy the Assumptions. Let $\mu_\phi$ be the unique equilibrium state for $f$ and $\phi$, and $m_\phi$ be as in Corollary~\ref{corMandMuUnique} and $\widetilde\phi$ as defined in (\ref{eqDefPhiTilde}). For each sequence $\{ x_n \}_{n\in\N}$ of points in $S^2$, we define the Borel probability measures
\begin{align}
         \nu_n & = \frac{1}{Z_n(\phi)} \sum\limits_{y\in f^{-n}(x_n)} \deg_{f^n} (y) \myexp\(S_n\phi(y)\) \delta_y,  \\
\widehat\nu_n & = \frac{1}{Z_n(\phi)} \sum\limits_{y\in f^{-n}(x_n)} \deg_{f^n} (y) \myexp\(S_n\phi(y)\) \frac{1}{n} \sum\limits_{i=0}^{n-1} \delta_{f^i(y)},\\
         \widetilde\nu_n & = \frac{1}{Z_n\big(\widetilde\phi \hspace{0.5mm} \big)} \sum\limits_{y\in f^{-n}(x_n)} \deg_{f^n} (y) \myexp\bigl(S_n\widetilde\phi(y)\bigr) \delta_y, 
\end{align}
for each $n\in\N_0$, where $Z_n(\psi) = \sum\limits_{y\in f^{-n}(x_n)} \deg_{f^n} (y) \myexp\(S_n\psi(y)\)$, for $\psi\in\CCC(S^2)$. Then
\begin{equation}  \label{eqWeakConvPreImgToMWithWeight}
\nu_n \stackrel{w^*}{\longrightarrow} m_\phi \text{ as } n\longrightarrow +\infty,
\end{equation}
\begin{equation}  \label{eqWeakConvPreImgToMuSumWithWeight}
\widehat\nu_n \stackrel{w^*}{\longrightarrow} \mu_\phi \text{ as } n\longrightarrow +\infty,
\end{equation}
\begin{equation}  \label{eqWeakConvPreImgToMuTildeWithWeight}
\widetilde\nu_n \stackrel{w^*}{\longrightarrow} \mu_\phi \text{ as } n\longrightarrow +\infty.
\end{equation}
\end{prop}

We note that when $\phi \equiv 0$ and $x_n=x_{n+1}$ for each $n\in\N$, the versions (\ref{eqWeakConvPreImgToMWithWeight}) and (\ref{eqWeakConvPreImgToMuTildeWithWeight}) reduce to (1.2) of Theorem~1.2 in \cite{Li13}.



\begin{proof}
We note that (\ref{eqWeakConvPreImgToMuSumWithWeight}) follows directly from Lemma~\ref{lmDerivConv}.

The proof of (\ref{eqWeakConvPreImgToMWithWeight}) is similar to that of Lemma~\ref{lmDerivConv}. For the completeness, we include it here in detail.

For each sequence $\{x_n\}_{n\in\N}$ of points in $S^2$, and each $u\in\CCC(S^2,d)$, by (\ref{eqR^nExpr}) and (\ref{eqDefR-}) we have
\begin{equation*}
  \langle \nu_n, u \rangle 
=  \frac{\RR^n_\phi (u)(x_n)}{\RR^n_\phi (\mathbbm{1})(x_n)}  
= \frac{\RR^n_{\overline\phi} (u)(x_n)}{\RR^n_{\overline\phi} (\mathbbm{1})(x_n)}.
\end{equation*}
By Theorem~\ref{thmRR^nConv},
\begin{equation*}
\Norm{\RR^n_{\overline\phi}(\mathbbm{1}) - u_\phi }_\infty  \longrightarrow  0 \text{ and }\Norm{\RR^n_{\overline\phi}(u) - u_\phi \int \! u \, \mathrm{d} m_\phi }_\infty  \longrightarrow  0
\end{equation*}
as $n\longrightarrow +\infty$. So by (\ref{eqU_phiBounds}),
\begin{equation*}
\lim\limits_{n\to+\infty} \frac{\RR^n_{\overline\phi} (u)(x_n)}{\RR^n_{\overline\phi} (\mathbbm{1})(x_n)} = \int \! u \, \mathrm{d}m_\phi.
\end{equation*}
Hence, (\ref{eqWeakConvPreImgToMWithWeight}) holds.

Finally, (\ref{eqWeakConvPreImgToMuTildeWithWeight}) follows from (\ref{eqWeakConvPreImgToMWithWeight}) and the fact that $\widetilde\phi \in \Holder{\alpha}(S^2,d)$ (Lemma~\ref{lmTildePhiIsHolder}) and $m_{\widetilde\phi} = \mu_\phi$ (Corollary~\ref{corMandMuUnique}).
\end{proof}




For the rest of this section, we prove that almost surely,
$$
\frac{1}{n}\sum\limits_{i=0}^{n-1} \delta_{q_i}  \stackrel{w^*}{\longrightarrow} \mu_\phi \text{ as } n\longrightarrow +\infty,
$$
where $q_i \in S^2$, $i\in \N_0$, is the location of the $i$-th step of a certain random walk on $S^2$ induced by $\RR_{\widetilde\phi}$ starting from an arbitrary fixed starting position $q_0 \in S^2$. This result generalizes Theorem~7.1 of \cite{Li13}, which is Theorem~\ref{thmASConvToES} in the case when $\phi\equiv 0$.

More precisely, let $Q=\RR_{\widetilde\phi}$. Then for each $u\in\CCC(S^2)$,
$$
Qu(x) = \int \! u(y) \,\mathrm{d}\mu_x(y),
$$
where
$$
\mu_x = \sum\limits_{z\in f^{-1}(x)} \deg_f(z) \myexp\bigl( \widetilde\phi (z)\bigr) \delta_z.
$$
By (\ref{eqRtildePhi1=1}), we get that $\mu_x\in\PPP(S^2)$ for each $x\in S^2$. We showed that the Ruelle operator in (\ref{eqDefRuelleOp}) is well-defined, from which it immediately follows that the map $x\mapsto \mu_x$ from $S^2$ to $\PPP(S^2)$ is continuous with respect to weak$^*$ topology on $\PPP(S^2)$. The operator $Q$ (or equivalently, the measures $\mu_x$, $x\in S^2$) and an arbitrary starting point $q_0\in S^2$ determine a random walk $\{q_i\}_{i\in\N_0}$ on $S^2$ with the probability that $q_{i+1}\in A$ is equal to $\mu_{q_i}(A)$ for each $i\in\N_0$ and each Borel set $A\subseteq S^2$. In the language of \cite[Section~8]{Li13}, this random walk is a \emph{Markov process determined by the operator $Q$}. We refer the reader to \cite[Section~8]{Li13} for a more detailed discussion.

\begin{theorem}    \label{thmASConvToES}
Let $f$, $d$, $\phi$, $\alpha$ satisfy the Assumptions. Let $\mu_\phi$ be the unique equilibrium state for $f$ and $\phi$, and $\widetilde\phi$ be as defined in (\ref{eqDefPhiTilde}). Suppose that $q_0\in S^2$ and $\{q_i\}_{i\in\N_0}$ is the random walk determined by $Q=\RR_{\widetilde\phi}$ described above. Then almost surely,
$$
\frac{1}{n}\sum\limits_{i=0}^{n-1} \delta_{q_i}  \stackrel{w^*}{\longrightarrow} \mu_\phi \text{ as } n\longrightarrow +\infty.
$$
\end{theorem}

\begin{proof}
By Corollary~\ref{corMandMuUnique}, the equilibrium state $\mu_\phi$ is the unique Borel probability measure on $S^2$ that satisfies $Q^*(\mu_\phi)=\mu_\phi$. Then the theorem follows directly from a theorem of H.~Furstenberg and Y.~Kifer in \cite{FK83} formulated as Theorem~7.2 in \cite{Li13}.
\end{proof}

























==> section/Spectral_gap.tex <==
% !TEX root = ../main.tex

\section{Normalized split Ruelle operators and spectral gap}
\label{sec:Normalized split Ruelle operators and spectral gap}


This section is devoted to the uniqueness of the equilibrium states for subsystems. 
We first define normalized split Ruelle operators and obtain some basic properties in Subsection~\ref{sub:Normalized split Ruelle operators}. 
Then in Subsection~\ref{sub:Convergence estimates} we introduce the notion of abstract modulus of continuity and establish various estimates for functions under normalized split Ruelle operators. 
Our goal in Subsection~\ref{sub:Uniqueness} is to prove the following statement. 


\subsection{Normalized split Ruelle operators}%
\label{sub:Normalized split Ruelle operators}

In this subsection we define normalized split Ruelle operators and establish some basic properties.

\smallskip

Let $f \colon S^2 \mapping S^2$ be an expanding Thurston map with a Jordan curve $\mathcal{C}\subseteq S^2$ satisfying $\post{f} \subseteq \mathcal{C}$ and $f(\mathcal{C}) \subseteq \mathcal{C}$. 
Let $d$ be a visual metric for $f$ on $S^2$, and $\phi \in C^{0,\holderexp}(S^2,d)$ a real-valued \holder continuous function with an exponent $\holderexp \in (0,1]$. 
Let $\juxtapose{X^0_{\black}}{X^0_{\white}} \in \mathbf{X}^0(f, \mathcal{C})$ be the black $0$-tile and the white $0$-tile, respectively. 
Recall from Definition~\ref{def:split sphere} and Remark~\ref{rem:disjoint union} that $\splitsphere = X^0_{\black} \sqcup X^0_{\white}$ is the disjoint union of $X^0_{\black}$ and $X^0_{\white}$, and the product spaces $\splfunspace$, $\splboufunspace$, and $\splmeaspace$ are identified with $C(\splitsphere)$, $B(\splitsphere)$, and $\mathcal{M}(\splitsphere)$, respectively. 


Let $F \in \subsystem$ be strongly primitive and $\eigfun = \splfun \in C(\splitsphere)$ be the continuous function given by Theorem~\ref{thm:existence of f invariant Gibbs measure}.
Note that $\eigfun(\widetilde{x}) > 0$ for each $\widetilde{x} \in \splitsphere = \disjointuniontile$ by \eqref{eq:two sides bounds for eigenfunction} in Theorem~\ref{thm:existence of f invariant Gibbs measure}.
Recall that by \eqref{eq:def:normed potential} and Theorem~\ref{thm:subsystem characterization of pressure},
\[
    \normpotential = \phi - \pressure.
\]

For each $n \in \n_0$ and each pair of $\juxtapose{\colour}{\colour'} \in \colours$, we define a map $\toperator{n}{\colour}{\colour'} \colon \boufunspace{\colour'} \mapping B(X^{0}_{\colour})$ by
\begin{equation}    \label{eq:def:twisted partial Ruelle operator}
    \begin{split}
        \toperator{n}{\colour}{\colour'}(v)(x) 
        &\define \sum_{ y \in F^{-n}(x) } \ccndegF{\colour}{\colour'}{n}{y} v(y) \myexp[\big]{ S_{n}^{F}\phi(y) - n\pressure + \log u_{\colour'}(y) - \log u_{\colour}(x) }  \\
        &= \sum_{ \substack{ y = (F^{n}|_{X^n})^{-1}(x) \\ X^n \in \ccFTile{n}{\colour}{\colour'}} } v(y) \myexp[\big]{ S_{n}^{F}\phi(y) - n\pressure + \log u_{\colour'}(y) - \log u_{\colour}(x) }
    \end{split}
\end{equation}
for each $v \in \boufunspace{\colour'}$ and each point $x \in X^0_{\colour}$. 
Similar to Lemma~\ref{lem:well-defined partial Ruelle operator}, for all $\juxtapose{n}{k} \in \n_0$, $\juxtapose{\colour}{\colour'} \in \colours$, and $v \in \confunspace{\colour'}$, we have
\begin{equation}    \label{eq:well-defined continuity of twisted partial Ruelle operator}
    \, \toperator{n}{\colour}{\colour'} (v) \in C\bigl(X^{0}_{\colour}\bigr) \qquad\qquad \text{and }
\end{equation}
\begin{equation}    \label{eq:iteration of twisted partial Ruelle operator}
    \qquad \qquad  \toperator{n + k}{\colour}{\colour'} (v) = \sum_{\colour'' \in \colours} \toperator{n}{\colour}{\colour''} \bigl( \toperator{k}{\colour''}{\colour'}(v) \bigr).
\end{equation}

Note that by \eqref{eq:definition of partial Ruelle operators} in Definition~\ref{def:partial Ruelle operator}, we can write the left hand side of \eqref{eq:def:twisted partial Ruelle operator} as
\begin{equation}\label{eq:equivalent definition of twisted partial Ruelle operator}
    \begin{aligned}        
        \toperator{n}{\colour}{\colour'}(v)(x) 
        &= \frac{1}{u_{\colour}(x)} \sum_{ X^n \in \ccFTile{n}{\colour}{\colour'} } 
        (u_{\colour'} \cdot v) \bigl((F^{n}|_{X^n})^{-1}(x) \bigr) \myexp[\big]{ S_{n}^{F}\phi\bigl( (F^{n}|_{X^n})^{-1}(x) \bigr) -n\pressure } \\
        &= \frac{1}{u_{\colour}(x)} \poperator[\normpotential]{n}(u_{\colour'} v)(x).
    \end{aligned}
\end{equation}

\begin{definition}[Normalized Split Ruelle operators]    \label{def:normalized split ruelle operator}
    Let $f$, $\mathcal{C}$, $F$, $d$, $\phi$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive. 
    Let $\eigfun = \splfun \in C(\splitsphere)$ be the continuous function given by Theorem~\ref{thm:existence of f invariant Gibbs measure}. 
    The \emph{normalized split Ruelle operator} $\twistsplopt \colon \splfunspace \mapping \splfunspace$ for the subsystem $F$ and potential $\phi$ is defined by
    \begin{equation}    \label{eq:def:normalized split Ruelle operator expand form}
        \twistsplopt\splfunv \define \bigl( 
            \toperator{1}{\black}{\black}(u_{\black}) + \toperator{1}{\black}{\white}(u_{\white}), 
            \toperator{1}{\white}{\black}(u_{\black}) + \toperator{1}{\white}{\white}(u_{\white})
        \bigr)
    \end{equation}
    for each $v_{\black} \in C\bigl(X^0_{\black}\bigr)$ and each $v_{\white} \in C\bigl(X^0_{\white}\bigr)$, or equivalently, $\twistsplopt \colon C(\splitsphere) \mapping C(\splitsphere)$ is defined by 
    \begin{equation}    \label{eq:def:normalized split Ruelle operator}
        \twistsplopt(\widetilde{v}) \define \frac{1}{\eigfun} \normsplopt(\eigfun \widetilde{v} )
    \end{equation} 
    for each $\widetilde{v} \in C(\splitsphere)$.    
\end{definition}

Note that by \eqref{eq:def:twisted partial Ruelle operator} and \eqref{eq:well-defined continuity of twisted partial Ruelle operator}, the normalized split Ruelle operator $\twistsplopt$ is well-defined, and the equivalence of two definitions \eqref{eq:def:normalized split Ruelle operator expand form} and \eqref{eq:def:normalized split Ruelle operator} follows from \eqref{eq:equivalent definition of twisted partial Ruelle operator} and Definition~\ref{def:split ruelle operator}.
By \eqref{eq:def:twisted partial Ruelle operator}, $\twistsplopt^{0}$ is the identity map on $C(\splitsphere)$.
Moreover, one sees that $\twistsplopt \colon \splfunspace \mapping \splfunspace$ has a natural extension to the space $\splboufunspace$ given by \eqref{eq:def:normalized split Ruelle operator expand form} for each $v_{\black} \in B\bigl(X^0_{\black}\bigr)$ and each $v_{\white} \in B\bigl(X^0_{\white}\bigr)$. % Moreover, by holder, splitoperator is hold Holder.

We show that the normalized split Ruelle operator $\twistsplopt$ is well-behaved under iterations.

\begin{lemma}    \label{lem:iteration of normalized split ruelle operator}
    Let $f$, $\mathcal{C}$, $F$, $d$, $\phi$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive. 
    Then for all $n \in \n_0$ and $\widetilde{v} = \splfunv \in C(\splitsphere)$, we have
    \begin{equation}    \label{eq:iteration of normalized split ruelle operator}
        \twistsplopt^{n}(\widetilde{v}) = \frac{1}{\eigfun} \normsplopt^{n}(\eigfun \widetilde{v} ) \qquad\quad \text{ and }
    \end{equation}
    \begin{equation}    \label{eq:iteration of normalized split ruelle operator expand form}
        \twistsplopt^{n} \splfunv = \bigl( \toperator{n}{\black}{\black}(v_{\black}) + \toperator{n}{\black}{\white}(v_{\white}), \
        \toperator{n}{\white}{\black}(v_{\black}) + \toperator{n}{\white}{\white}(v_{\white}) \bigr).
    \end{equation}
\end{lemma}
\begin{proof}
    It follows immediately from \eqref{eq:def:normalized split Ruelle operator} and Definition~\ref{def:split ruelle operator} that \eqref{eq:iteration of normalized split ruelle operator} holds for all $n \in \n$. 
    Since $F$ is surjective, i.e., $F(\domF) = S^{2}$, we know that $\splopt^{0}$ is the identity map on $C(\splitsphere)$ by Definition~\ref{def:split ruelle operator}. 
    Thus \eqref{eq:iteration of normalized split ruelle operator} also holds for $n = 0$.

    The case where $n = 0$ and the case where $n = 1$ both hold by definition. 
    Assume now \eqref{eq:iteration of normalized split ruelle operator expand form} holds for $n = k$ for some $k \in \n$. 
    Then by Definition~\ref{def:normalized split ruelle operator} and \eqref{eq:iteration of twisted partial Ruelle operator}, for each $\colour \in \colours$ we have
    \begin{align*}
    \pi_{\colour}\bigl( \twistsplopt^{k + 1}\splfunv \bigr) 
        &= \pi_{\colour}\bigl( 
            \twistsplopt\bigl( 
                \toperator{k}{\black}{\black}(v_{\black}) + \toperator{k}{\black}{\white}(v_{\white}), \
                \toperator{k}{\white}{\black}(v_{\black}) + \toperator{k}{\white}{\white}(v_{\white}) 
            \bigr) 
        \bigr) \\
        &= \sum_{\colour' \in \colours} \toperator{1}{\colour}{\colour'} \bigl( 
                \toperator{k}{\colour'}{\black}(v_{\black}) + \toperator{k}{\colour'}{\white}(v_{\white}) 
            \bigr)  \\
        &= \sum_{\colour'' \in \colours} \sum_{\colour' \in \colours} \toperator{1}{\colour}{\colour'} \bigl( \toperator{k}{\colour'}{\colour''}(v_{\colour''}) \bigr)  
        = \sum_{\colour'' \in \colours} \toperator{k + 1}{\colour}{\colour''}(v_{\colour''}),
    \end{align*}
    for $v_{\black} \in C\bigl(X^0_{\black}\bigr)$ and $v_{\white} \in C\bigl(X^{0}_{\white}\bigr)$. This completes the inductive step, establishing \eqref{eq:iteration of normalized split ruelle operator expand form}.
\end{proof}

\begin{rmk}
    Similarly, one can show that \eqref{eq:iteration of normalized split ruelle operator} and \eqref{eq:iteration of normalized split ruelle operator expand form} holds for $\widetilde{v} = \splfunv \in \splboufunspace$.
\end{rmk}

Recall $\spleigmea \in \probmea{\splitsphere}$ from Theorem~\ref{thm:subsystem:eigenmeasure existence and basic properties}. 
Then we can show that $\splmea = \eigfun \spleigmea \in \probmea{\splitsphere}$ defined in Theorem~\ref{thm:existence of f invariant Gibbs measure} satisfies
\begin{equation}  \label{eq:equilibrium state is eigenmeasure of dual normalized split operator}
    \dualtwistsplopt\splmea = \splmea,
\end{equation}
where $\dualtwistsplopt$ is the adjoint operator of $\twistsplopt$ on the space $\splmeaspace$.
Indeed, by \eqref{eq:def:normalized split Ruelle operator} and \eqref{eq:eigenmeasure for dual split operator}, for $\widetilde{v} \in C(\splitsphere)$,
\begin{align*}
    \functional[\big]{\dualtwistsplopt\splmea}{\widetilde{v}} 
    &= \functional[\big]{\eigfun\spleigmea}{\twistsplopt(\widetilde{v})} = \functional[\big]{\spleigmea}{ \normsplopt(\eigfun \widetilde{v})} \\
    &= \functional[\big]{ \normdualsplopt\spleigmea}{\eigfun \widetilde{v}} = \functional{\spleigmea}{\eigfun \widetilde{v}} = \functional{\splmea}{\widetilde{v}}.
\end{align*}

Recall that we equip the spaces $C(\splitsphere)$ and $\splfunspace$ with the uniform norm given by\[
    \normcontinuous{\widetilde{v}}{\splitsphere} = \norm{\splfunv} 
    = \max \bigl\{ \normcontinuous{v_{\black}}{X^0_{\black}}, \normcontinuous{v_{\white}}{X^{0}_{\white}} \bigr\}
\] for $\widetilde{v} = \splfunv \in \splfunspace$.

\begin{lemma}   \label{lem:norm of normalized split operator}
    Let $f$, $\mathcal{C}$, $F$, $d$, $\phi$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive.
    Then the operator norm of $\twistsplopt$ is given by $\normcontinuous[\big]{\twistsplopt}{\splitsphere} = 1$. 
    In addition, $\twistsplopt\bigl(\indicator{\splitsphere}\bigr) = \indicator{\splitsphere}$.
\end{lemma}
\begin{proof}
    By Definition~\ref{def:normalized split ruelle operator}, \eqref{eq:eigenfunction of normed split operator}, and \eqref{eq:def:twisted partial Ruelle operator}, \[
        \twistsplopt\bigl(\indicator{\splitsphere}\bigr) = \frac{1}{\eigfun} \normsplopt(\eigfun) = \indicator{\splitsphere},
    \]
    i.e., for each $\widetilde{x} = (x, \colour) \in \splitsphere$,
    \[
        \begin{split}
            1 = \sum_{\colour' \in \colours} \sum_{ X^1 \in \ccFTile{1}{\colour}{\colour'} } \myexp[\big]{ \phi ( x_{X^{1}} ) - \pressure + \log u_{\colour'} ( x_{X^{1}} ) - \log u_{\colour}(x) },
        \end{split}
    \]
    where we write $x_{X^{1}} \define (F|_{X^{1}})^{-1}(x)$ for $X^1 \in \ccFTile{1}{\colour}{\colour'}$. 
    Then for each $\widetilde{x} = (x, \colour) \in \splitsphere$ and each $\widetilde{v} = \splfunv \in \splfunspace$, we have
    \begin{align*}
        \Bigl| \twistsplopt(\widetilde{v})(\widetilde{x}) \Bigl|
        &= \bigg| \sum_{\colour' \in \colours} \sum_{  X^1 \in \ccFTile{1}{\colour}{\colour'} } v_{\colour'}( x_{X^{1}} ) \myexp[\big]{ \phi( x_{X^{1}} ) - \pressure + \log u_{\colour'}( x_{X^{1}} ) - \log u_{\colour}(x) } \bigg|  \\
        &\leqslant \normcontinuous{\widetilde{v}}{\splitsphere}  \abs[\bigg]{ \sum_{\colour' \in \colours} \sum_{ X^1 \in \ccFTile{1}{\colour}{\colour'} } \myexp[\big]{ \phi( x_{X^{1}} ) - \pressure + \log u_{\colour'}( x_{X^{1}} ) - \log u_{\colour}(x) } }  \\
        &= \normcontinuous{\widetilde{v}}{\splitsphere}.
    \end{align*}
    Thus $\normcontinuous[\big]{\twistsplopt}{\splitsphere} \leqslant 1$. Since $\twistsplopt\bigl(\indicator{\splitsphere}\bigr) = \indicator{\splitsphere}$, we get $\normcontinuous[\big]{\twistsplopt}{\splitsphere} = 1$.
\end{proof}

% normalized potential is holder
% \begin{lemma}  \label{lmTildePhiIsHolder}
% Let $f$, $d$, $\phi$, $\alpha$ satisfy the Assumptions. Then
% \begin{equation}  \label{eqTildePhiIsHolder}
% \widetilde\phi \in \Holder{\alpha}(S^2,d).
% \end{equation}
% \end{lemma}

% \begin{proof}
% By Theorem~\ref{thmMuExist}, $u_\phi \in \Holder{\alpha}(S^2,d)$ and $C_2^{-1} \leq u_\phi (x) \leq C_2$ for each $x\in S^2$, where $C_2\geq 1$ is the constant from Lemma~\ref{lmSigmaExpSnPhiBound}. So $\log u_\phi \in \Holder{\alpha}(S^2,d)$. Note that $\phi \in \Holder{\alpha}(S^2,d)$, so by (\ref{eqDefPhiTilde}) it suffices to show that $u_\phi \circ f \in \Holder{\alpha}(S^2,d)$. But this follows from the fact that $f$ is Lipschitz with respect to $d$ (Lemma~\ref{lmLipschitz}) and $u_\phi \in \Holder{\alpha}(S^2,d)$.
% \end{proof}










\subsection{Spectral gap}%
\label{sub:Convergence estimates}

% abstract modulus of continuity
Let $(X, d)$ be a metric space. A function $\modufun \colon [0, +\infty) \mapping [0, +\infty)$ is an \emph{abstract modulus of continuity} if it is continuous at $0$, non-decreasing, and $\modufun(0) = 0$.  
Given any constant $\moduconst \in [0, +\infty]$ and any abstract modulus of continuity $\modufun$, we define the subclass $\moduspace$ of $C(X)$ as
\begin{align*}
    \moduspace \define \bigl\{ u \in C(X) \describe \uniformnorm{u} \leqslant \moduconst \text{ and for } \juxtapose{x}{y} \in S^2, \, \abs{u(x) - u(y)} \leqslant \modufun(d(x, y)) \bigr\}.
\end{align*}

Assume now that $(X, d)$ is compact. Then by the \aalem Theorem, each $\moduspace$ is precompact in $C(X)$ equipped with the uniform norm. It is easy to see that each $\moduspace$ is compact. 
On the other hand, for $v \in C(X)$, we can define an abstract modulus of continuity by
\begin{equation}    \label{eq:abstract modulus of continuity for continuous function}
    \modufun(t) = \sup \{ \abs{v(x) - v(y)} \describe \juxtapose{x}{y} \in X, \, d(x, y) \leqslant t \}
\end{equation}
for $t \in [0, +\infty)$, so that $v \in \moduspace[\iota]$, where $\iota = \uniformnorm{v}$.

The following lemma is easy to check (see also \cite[Lemma~5.24]{li2017ergodic}).
\begin{lemma}    \label{lem:product and inverse of modulus of continuity}
    Let $(X, d)$ be a metric space. 
    For all constants $\moduconst > 0$, $\moduconst_1, \, \moduconst_2 \geqslant 0$ and abstract moduli of continuity $\modufun_1, \, \modufun_2$, we have
    \[
        \begin{split}
            \bigl\{ v_1 v_2 \describe v_1 \in \moduspace[\moduconst_{1}][\modufun_{1}], \, v_2 \in \moduspace[\moduconst_{2}][\modufun_{2}] \bigr\} &\subseteq \moduspace[\moduconst_{1}\moduconst_{2}][\moduconst_{1}\modufun_{2} + \moduconst_{2}\modufun_{1}], \\
            \bigl\{ 1 / v \describe v \in \moduspace[\moduconst_{1}][\modufun_{1}] , \, v(x) \geqslant \moduconst \text{ for each } x \in X \bigr\}  &\subseteq \moduspace[\moduconst^{-1}][\moduconst^{-2} \modufun_{1}] .
        \end{split}
    \]    
\end{lemma}


\begin{proposition}   \label{prop:modulus for function under split ruelle operator}
    Let $f$, $\mathcal{C}$, $F$, $d$, $\Lambda$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive.
    %Let $f \colon S^2 \rightarrow S^2$ be an expanding Thurston map, and $d$ be a visual metric on $S^2$ for $f$ with an expansion factor $\Lambda>1$ and a linear local connectivity constant $L\geq 1$. 
    Then for each $\holderexp \in (0,1]$, each $\moduconst \geqslant 0$, and each $K \geqslant 0$, there exist constants $\widehat{\moduconst} \geqslant 0$ and $\widehat{C} \geqslant 0$ with the following property:

    For each abstract modulus of continuity $\modufun$, there exists an abstract modulus of continuity $\widetilde{\modufun}$ such that for each $\potential \in \holderspacesphere$ with $\holdernorm{\phi}{S^2} \leqslant K$, we have
    \begin{align}
        \label{eq:modulus for function under normed split Ruelle operator}
        \bigl\{ \normsplopt^{n}(\widetilde{v}) \describe \widetilde{v} = \splfunv \in \splmoduspace, \, n \in \n_0 \bigr\} &\subseteq \splmoduspace[\widehat{\moduconst}][\widehat{\modufun}],  \\
        \label{eq:modulus for function under normalized split Ruelle operator}
        \bigl\{ \twistsplopt^{n}(\widetilde{v}) \describe \widetilde{v} = \splfunv \in \splmoduspace, \, n \in \n_0 \bigr\} &\subseteq \splmoduspace[\moduconst][\widetilde{\modufun}],
    \end{align}
    % \begin{equation}   \label{eq:modulus for function under normed split Ruelle operator}
    %     \bigl\{ \normsplopt^{n}(\widetilde{v}) \describe \widetilde{v} = \splfunv \in \splmoduspace, \, n \in \n_0 \bigr\} \subseteq \splmoduspace[\widehat{\moduconst}][\widehat{\modufun}],
    % \end{equation}   
    % \begin{equation}   \label{eq:modulus for function under normalized split Ruelle operator}
    %     \Bigl\{ \twistsplopt^{n}(\widetilde{v}) \describe \widetilde{v} = \splfunv \in \splmoduspace, \, n \in \n_0 \Bigr\} \subseteq \splmoduspace[\moduconst][\widetilde{\modufun}],
    % \end{equation}
    where $\widehat{\modufun}(t) \define \widehat{C}\bigl(t^{\holderexp} + \modufun(C_0 t)\bigr)$ is an abstract modulus of continuity, and $C_0 > 1$ is the constant depending only on $f$, $\mathcal{C}$, and $d$ from Lemma~\ref{lem:basic_distortion}.
\end{proposition}
\begin{proof}
    Fix arbitrary $\holderexp \in (0,1]$, $\moduconst \geqslant 0$, and $K \geqslant 0$. 
    By Lemma~\ref{lem:iteration of split-partial ruelle operator} and \eqref{eq:second bound for normed split operator} in Lemma~\ref{lem:distortion lemma for normed split operator}, for all $n \in \n_0$, $\widetilde{v} = \splfunv \in \splmoduspace$, and $\potential \in \holderspacesphere$ with $\holdernorm{\potential}{S^{2}} \leq K$, we have\[
        \normcontinuous[\big]{\normsplopt^{n}(\widetilde{v})}{\splitsphere} 
        \leqslant \normcontinuous{\widetilde{v}}{\splitsphere} \normcontinuous[\big]{\normsplopt^{n}(\indicator{\splitsphere})}{\splitsphere} 
        \leqslant \Csplratio \normcontinuous{\widetilde{v}}{\splitsphere},
    \]
    where $\Csplratio \geqslant 1$ is the constant defined in \eqref{eq:const:Csplratio} in Lemma~\ref{lem:distortion lemma for subsystem}~\ref{item:lem:distortion lemma for subsystem:uniform bound} and depends only on $F$, $\mathcal{C}$, $d$, $\phi$, and $\holderexp$.
    By \eqref{eq:const:Csplratio}, quantitatively,
    \[
        \Csplratio = \CsplratioExpression, 
    \]
    where $n_{F} \in \n$ is the constant depending only on $F$ and $\mathcal{C}$ in Definition~\ref{def:primitivity of subsystem} since $F$ is primitive, and $C_1 \geqslant 0$ is the constant defined in \eqref{eq:const:C_1} in Lemma~\ref{lem:distortion_lemma} depends only on $F$, $\mathcal{C}$, $d$, $\phi$, and $\holderexp$. 
    Quantitatively,\[
        C_1 = C_0 \frac{ \holderseminorm{\potential}{S^2} }{1 - \Lambda^{-\holderexp}},
    \]
    where $C_0 > 1$ is the constant depending only on $f$, $\mathcal{C}$, and $d$ in Lemma~\ref{lem:basic_distortion}.
    Let $C'_{1} \define \frac{ C_0 K }{1 - \Lambda^{-\holderexp}}$ and \[
        \Csplratio' \define (\deg{f})^{n_{F}} \myexp[\bigg]{ \frac{ C_0 K }{1 - \Lambda^{-\holderexp}} (\diam{d}{S^{2}} )^{\holderexp} + 2n_{F} K }.
    \]
    Then we have $C_1 \leqslant C'_1$ and $\Csplratio \leqslant \Csplratio'$ for each $\potential \in \holderspacesphere$ with $\holdernorm{\potential}{S^{2}} \leq K$.
    Note that both $C'_{1}$ and $\Csplratio'$ only depend on $F$, $\mathcal{C}$, $d$, $K$, and $\holderexp$. 
    Thus we can choose $\widehat{\moduconst} \define \Csplratio' \moduconst$. 

    For each $\colour \in \colours$ and each pair of $\juxtapose{x}{y} \in X^0_{\colour}$, we have 
    \begin{align*}
        &\quad\ \Big| \pi_{\colour}\bigl( \normsplopt^{n}\splfunv \bigl)(x) - \pi_{\colour}\bigl( \normsplopt^{n}\splfunv \bigl)(y) \Big|  \\
        &= \bigg| \paroperator[\normpotential]{n}{\colour}{\black}(v_{\black})(x) + \paroperator[\normpotential]{n}{\colour}{\white}(v_{\white})(x) 
            - \paroperator[\normpotential]{n}{\colour}{\black}(v_{\black})(y) - \paroperator[\normpotential]{n}{\colour}{\white}(v_{\white})(y)  \bigg| \\
        &\leqslant \sum_{\colour' \in \colours} \bigg| \paroperator[\normpotential]{n}{\colour}{\colour'}(v_{\colour})(x) - \paroperator[\normpotential]{n}{\colour}{\colour'}(v_{\colour})(y) \bigg|  \\
        &= \sum_{\colour' \in \colours} \Bigg| \sum_{X^n \in \ccFTile{n}{\colour}{\colour'}} 
            \bigl( v_{\colour'} \myexp[\big]{  S_n^{F}\normpotential } \bigr) \bigl( (F^{n}|_{X^{n}})^{-1}(x) \bigr) - \bigl( v_{\colour'} \myexp[\big]{ S_n^{F}\normpotential } \bigr) \bigl( (F^{n}|_{X^{n}})^{-1}(y) \bigr) \Bigg|   \\ % v_{\colour'} e^{ S_n^{F}\normpotential }
        &\leqslant \sum_{\colour' \in \colours} \Bigg| \sum_{X^n \in \ccFTile{n}{\colour}{\colour'}} 
            v_{\colour'}\bigl( (F^{n}|_{X^{n}})^{-1}(x) \bigr) \Bigl( e^{  S_n^{F}\normpotential( (F^{n}|_{X^{n}})^{-1}(x) ) } - e^{ S_n^{F}\normpotential( (F^{n}|_{X^{n}})^{-1}(y) ) } \Bigr)  \Bigg| \\
        &\qquad + \sum_{\colour' \in \colours} \Bigg| \sum_{X^n \in \ccFTile{n}{\colour}{\colour'}} 
            e^{ S_n^{F}\normpotential( (F^{n}|_{X^{n}})^{-1}(y) ) }   \Bigl( v_{\colour'}\bigl( (F^{n}|_{X^{n}})^{-1}(x) \bigr) - v_{\colour'}\bigl( (F^{n}|_{X^{n}})^{-1}(y) \bigr) \Bigr)  \Bigg|.
    \end{align*}
    The second term above is \[
        \leqslant \Csplratio \modufun(C_0 \Lambda^{-n} d(x, y)) \leqslant \Csplratio \modufun(C_0 d(x, y)) \leqslant \Csplratio' \modufun(C_0 d(x, y)),
    \]
    due to \eqref{eq:second bound for normed split operator} in Lemma~\ref{lem:distortion lemma for normed split operator} and the fact that $d\bigl( (F^{n}|_{X^{n}})^{-1}(x), (F^{n}|_{X^{n}})^{-1}(y) \bigr) \leqslant C_0 \Lambda^{-n} d(x, y)$ by Lemma~\ref{lem:basic_distortion}, where the constant $C_0$ comes from.

    To estimate the first term, we use the following general inequality for $s, t \in \real$,\[
        | \myexp{s} -\myexp{t} | \leqslant ( \myexp{s} + \myexp{t} ) ( \myexp{|s - t|} - 1).
    \]
    Then it follows from Lemma~\ref{lem:distortion_lemma}, Lemma~\ref{lem:iteration of split-partial ruelle operator}, and \eqref{eq:second bound for normed split operator} in Lemma~\ref{lem:distortion lemma for normed split operator} that the first term is 
    \begin{align*}
        &\leqslant \sum_{\colour' \in \colours} \sum_{X^n \in \ccFTile{n}{\colour}{\colour'}} \uniformnorm{v_{\colour'}} 
            \Bigl( e^{S_n^{F}\normpotential( (F^{n}|_{X^{n}})^{-1}(x) )} + e^{S_n^{F}\normpotential( (F^{n}|_{X^{n}})^{-1}(y) )} \Bigr)  \\
        &\qquad\qquad\qquad\qquad\qquad\qquad\!  \cdot \Bigl( e^{| S_n^{F}\normpotential( (F^{n}|_{X^{n}})^{-1}(x) ) - S_n^{F}\normpotential( (F^{n}|_{X^{n}})^{-1}(y) ) |} - 1 \Bigr)  \\
        &\leqslant \sum_{X^n \in \ccFTile{n}{\colour}{}} \moduconst \Bigl( e^{S_n^{F}\normpotential( (F^{n}|_{X^{n}})^{-1}(x) )} + e^{S_n^{F}\normpotential( (F^{n}|_{X^{n}})^{-1}(y) )} \Bigr) \bigl( \myexp[\big]{ C_1 d(x, y)^{\holderexp} } - 1\bigr) \\
        &\leqslant 2 \moduconst \Csplratio \bigl( \myexp[\big]{ C_1 d(x, y)^{\holderexp} } - 1\bigr) 
        \leqslant 2 \moduconst \Csplratio' \bigl( \myexp[\big]{ C'_{1} d(x, y)^{\holderexp} } - 1\bigr) 
        \leqslant 2 \moduconst \widetilde{C}_{1} d(x, y)^{\holderexp},
    \end{align*}
    for some constant $\widetilde{C}_{1} > 0$ that only depends on $C'_1$, $\Csplratio'$, and $\diam{d}{S^2}$.
    Here the justification of the third inequality above is similar to that of \eqref{eq:third bound for normed split operator} in Lemma~\ref{lem:distortion lemma for normed split operator}.
    Recall that both $C'_{1}$ and $\Csplratio'$ only depend on $F$, $\mathcal{C}$, $d$, $K$, and $\holderexp$, so does $\widetilde{C}_{1}$.

    Hence for each $\colour \in \colours$ and each pair of $\juxtapose{x}{y} \in X^0_{\colour}$, we have
     \[
        \Big| \pi_{\colour}\bigl( \normsplopt^{n}\splfunv \bigl)(x) - \pi_{\colour}\bigl( \normsplopt^{n}\splfunv \bigl)(y) \Big| \leqslant 
        \Csplratio' \modufun(C_0 d(x, y)) + 2 \moduconst \widetilde{C}_{1} d(x, y)^{\holderexp}.
    \]
    By choosing $\widehat{C} \define \max \bigl\{ \Csplratio', 2 \moduconst \widetilde{C}_{1} \bigr\}$, which only depends on $F$, $\mathcal{C}$, $d$, $K$, and $\holderexp$, we complete the proof of \eqref{eq:modulus for function under normed split Ruelle operator}.

    \smallskip

    We now prove \eqref{eq:modulus for function under normalized split Ruelle operator}.

    We fix an arbitrary $\potential \in \holderspacesphere$ with $\holdernorm{\potential}{S^{2}} \leq K$.
    Recall that $\eigfun = \splfun \in \splfunspace$ is a continuous function on $\splitsphere$ given by Theorem~\ref{thm:existence of f invariant Gibbs measure}. 
    Thus by \eqref{eq:two sides bounds for eigenfunction} in Theorem~\ref{thm:existence of f invariant Gibbs measure} we have\[
        \normcontinuous{\eigfun}{\splitsphere} \leqslant \moduconst_{1},
    \]
    where
    \[
        \moduconst_{1} \define \Csplratio' = (\deg{f})^{n_{F}} \myexp[\bigg]{ \frac{ C_0 K }{1 - \Lambda^{-\holderexp}} (\diam{d}{S^{2}} )^{\holderexp} + 2n_{F} K }.
    \]
    For each $\colour \in \colours$ and each pair of $\juxtapose{x}{y} \in X^0_{\colour}$, it follows from Theorem~\ref{thm:existence of f invariant Gibbs measure} and \eqref{eq:third bound for normed split operator} in Lemma~\ref{lem:distortion lemma for normed split operator} that 
    \begin{align*}
        | u_{\colour}(x) - u_{\colour}(y)| 
        &= \bigg| \lim_{n \to +\infty} \frac{1}{n} \sum_{j=0}^{n-1} \Bigl( \normsplopt^{j}\bigl(\indicator{\splitsphere}\bigr)(x, \colour) - \normsplopt^{j}\bigl(\indicator{\splitsphere}\bigr)(y, \colour) \Bigr)  \bigg| \\
        &\leqslant \limsup_{n \to +\infty} \frac{1}{n} \sum_{j=0}^{n-1} \Big| \normsplopt^{j}\bigl(\indicator{\splitsphere}\bigr)(x, \colour) - \normsplopt^{j}\bigl(\indicator{\splitsphere}\bigr)(y, \colour) \Big| \\
        &\leqslant \Csplratio \bigl( \myexp[\big]{ C_1 d(x, y)^{\holderexp} } - 1\bigr) 
        \leqslant \Csplratio' \bigl( \myexp[\big]{ C'_1 d(x, y)^{\holderexp} } - 1\bigr).
    \end{align*}
    Thus \[
        \eigfun = \splfun \in \splmoduspace[\moduconst_{1}][\modufun_{1}],
    \]
    where $\modufun_{1}$ is an abstract modulus of continuity defined by\[
        \modufun_{1}(t) \define \Csplratio' \bigl( \myexp[\big]{ C'_1 t^{\holderexp} } - 1\bigr), \quad \text{ for } t \in [0, +\infty).
    \]

    Thus it follows from Lemma~\ref{lem:product and inverse of modulus of continuity} that\[
        \begin{split}
            \bigl\{ \widetilde{v} \eigfun \describe \widetilde{v} = \splfunv & \in  \splmoduspace, \,  \potential \in \holderspacesphere, \, \holderseminorm{\potential}{S^2} \leqslant K \bigr\} \\
            &\subseteq \splmoduspace[\moduconst\moduconst_{1}][\moduconst\modufun_{1} + \moduconst_{1}\modufun].
        \end{split}
    \]
    Then by \eqref{eq:iteration of normalized split ruelle operator} in Lemma~\ref{lem:iteration of normalized split ruelle operator}, \eqref{eq:modulus for function under normed split Ruelle operator}, and Lemma~\ref{lem:product and inverse of modulus of continuity}, we get that there exists a constant $\widetilde{\moduconst} \geqslant 0$ and an abstract modulus of continuity $\widetilde{\modufun}$ such that for each $\potential \in \holderspacesphere$ with $\holderseminorm{\potential}{S^2} \leqslant K$, \[
        \bigl\{ \twistsplopt^{n}(\widetilde{v}) \describe \widetilde{v} = \splfunv \in \splmoduspace, \, n \in \n_0 \bigr\} \subseteq \splmoduspace[\widetilde{\moduconst}][\widetilde{\modufun}].
    \] 

    On the other hand, by Lemma~\ref{lem:norm of normalized split operator}, $\normcontinuous[\big]{\twistsplopt^{n}(\widetilde{v})}{\splitsphere} \leqslant \normcontinuous{\widetilde{v}}{\splitsphere} \leqslant \widetilde{\moduconst}$ for each $\widetilde{v} = \splfunv \in \splmoduspace$, each $n \in \n_0$, and each $\potential \in \holderspacesphere$. 
    Therefore, we have proved \eqref{eq:modulus for function under normalized split Ruelle operator}.
\end{proof}


We now establish a generalization of \cite[]{} 

\begin{lemma}    \label{lem:upper bound for uniform norm of normalized split ruelle operator}
    Let $f$, $\mathcal{C}$, $F$, $d$, $\Lambda$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive.
    Let $\modufun$ be an abstract modulus of continuity. 
    Then for each $\holderexp \in (0,1]$, each $K \in [0 +\infty)$, and each $\delta_{1} \in (0, +\infty)$, there exist constants $\delta_2 \in (0, +\infty)$ and $N \in \n$ with the following property:

    For each $\widetilde{v} = \splfunv \in \splmoduspace[+\infty]$, each $\potential \in \holderspacesphere$, and each choice of $\spleigmea \in \probmea{\splitsphere}$ from Theorem~\ref{thm:subsystem:eigenmeasure existence and basic properties}, if $\holdernorm{\potential}{S^2} \leqslant K$, $\normcontinuous{\widetilde{v}}{\splitsphere} \geqslant \delta_1$, and $\int \! \widetilde{v}\eigfun \,\mathrm{d}\spleigmea = 0$, then\[
        \normcontinuous[\big]{\twistsplopt^{N}(\widetilde{v})}{\splitsphere} \leqslant \normcontinuous{\widetilde{v}}{\splitsphere} - \delta_2.
    \]
\end{lemma}
\begin{rmk}
    Note that at this point, we have yet to prove that $\spleigmea$ from Theorem~\ref{thm:subsystem:eigenmeasure existence and basic properties} is unique. We will prove it in Proposition~\ref{prop:uniqueness of eigenmeasure subsystem}. Recall that $\eigfun = \splfun \in C(\splitsphere)$ is defined in Theorem~\ref{thm:existence of f invariant Gibbs measure} that depends only on $F$, $\mathcal{C}$, and $\potential$. 
\end{rmk}
\begin{proof}
    Fix arbitrary constants $\holderexp \in (0, 1]$, $K \in [0, +\infty)$, and $\delta_1 \in (0, +\infty)$. 
    Fix $\epsilon > 0$ sufficiently small such that $\modufun(\epsilon) < \delta_{1}/2$. Then $\epsilon$ depends only on $\modufun$ and $\delta_{1}$.
    Fix a choice of $\spleigmea \in \probmea{\splitsphere}$ from Theorem~\ref{thm:subsystem:eigenmeasure existence and basic properties}, an arbitrary $\potential \in \holderspacesphere$, and an arbitrary $\widetilde{v} = \splfunv \in \splmoduspace[+\infty]$ with $\holdernorm{\potential}{S^2} \leqslant K$, $\normcontinuous{\widetilde{v}}{\splitsphere} \geqslant \delta_1$, and $\int \! \widetilde{v}\eigfun \,\mathrm{d}\spleigmea = 0$.

    Let $\spllimitset$ be the subset of $\splitsphere$ defined by 
    \[
        \spllimitset \define \bigcap\limits_{n \in \n} \bigcup \splDomain{n},
    \]
    where
    \[
        \splDomain{n} \define  \bigcup_{\colour \in \colours} \bigl\{ i_{\colour}(X^n) \describe X^n \in \Domain{n}, \, X^n \subseteq X^0_{\colour} \bigr\}.
    \]
    Recall that $i_{\colour}$ is defined by \eqref{eq:natural injection into splitsphere}. 
    Mimicking the proofs of Proposition~\ref{prop:dual split operator}~\ref{item:prop:dual split operator:measure concentrate} and Theorem~\ref{thm:subsystem:eigenmeasure existence and basic properties}~\ref{item:thm:subsystem:eigenmeasure existence and basic properties:eigenmeasure support on limitset}, we can show that $\spleigmea \bigl(\widetilde{\limitset} \bigr) = 1$. We postpone its proof to the end of this proof. 
    
    Since $\spleigmea \in \probmea{\splitsphere}$ supports on $\widetilde{\limitset}$ and $\int \! \widetilde{v}\eigfun \,\mathrm{d}\spleigmea = 0$, there exist points $\widetilde{y}_{-}, \, \widetilde{y}_{+} \in \widetilde{\limitset}$ such that $\widetilde{v}(\widetilde{y}_{-}) \leqslant 0$ and $\widetilde{v}(\widetilde{y}_{+}) \geqslant 0$. 
    By Definition~\ref{def:split sphere}, we have $\widetilde{y}_{-} = (y_{-}, \colour')$ for some $\colour' \in \colours$ and $y_{-} \in X^0_{\colour'}$, and $\widetilde{y}_{+} = (y_{+}, \colour'')$ for some $\colour'' \in \colours$ and $y_{+} \in X^0_{\colour''}$.

    We fix an arbitrary point $\widetilde{x} \in \splitsphere$. 
    Then there exist $\colour \in \colours$ and $x \in X^0_{\colour}$ satisfying $\widetilde{x} = (x, \colour)$. 

    Since $\widetilde{y}_{-} = (y_{-}, \colour') \in \widetilde{\limitset}$, it follows from the definition of $\widetilde{\limitset}$ that there exists a sequence of tiles $\{ X^{n} \}_{n \in \n}$ satisfying $X^n \in \Domain{n}$ and $y_{-} \in X^{n + 1} \subseteq X^n \subseteq X^0_{\colour'}$ for each $n \in \n$. 
    By Lemma~\ref{lem:visual_metric}~\ref{item:lem:visual_metric:diameter of cell}, there exists an integer $n_{\epsilon} \in \n$ depending only on $F$, $\mathcal{C}$, $d$, $\modufun$, and $\delta_{1}$ such that $\diam{d}{Y^{n_{\epsilon}}} < \epsilon$ for each $n_{\epsilon}$-tile $Y^{n_{\epsilon}} \in \Tile{n_{\epsilon}}$.
    Thus we have $y_{-} \in X^{n_{\epsilon}} \subseteq B_{d}(y_{-}, \epsilon) \cap X^0_{\colour'}$. 
    By Proposition~\ref{prop:subsystem:properties}~\ref{item:subsystem:properties:homeo}, we have $X^0 \define F^{n_{\epsilon}}(X^{n_{\epsilon}}) \in \bigl\{ \blacktile, \whitetile \bigr\}$. 
    Since $F \in \subsystem$ is primitive, by Definition~\ref{def:primitivity of subsystem}, there exist $n_{F} \in \n$ and $Y^{n_{F}} \in \Domain{n_{F}}$ satisfying $Y^{n_{F}} \subseteq X^0$ and $F^{n_{F}}(Y^{n_{F}}) = X^0_{\colour}$. 
    Then it follows from Lemma~\ref{lem:cell mapping properties of Thurston map}~\ref{item:lem:cell mapping properties of Thurston map:i} and Proposition~\ref{prop:subsystem:properties}~\ref{item:subsystem:properties:homeo} that $Y^{n_{\epsilon} + n_{F}} \define \bigl(F^{n_{\epsilon}}|_{X^{n_{\epsilon}}}\bigr)^{-1}(Y^{n_{F}}) \in \Domain{n_{\epsilon} + n_{F}}$. 
    Note that $Y^{n_{\epsilon} + n_{F}} \subseteq X^{n_{\epsilon}} \subseteq X^0_{\colour'}$ and $F^{n_{\epsilon} + n_{F}}(Y^{n_{\epsilon} + n_{F}}) = F^{n_{F}}(Y^{n_{F}}) = X^0_{\colour}$. 
    Thus $Y^{n_{\epsilon} + n_{F}} \in \ccFTile{n_{\epsilon} + n_{F}}{\colour}{\colour'}$.
    Set $y \define \bigl(F^{n_{\epsilon} + n_{F}}|_{Y^{n_{\epsilon} + n_{F}}}\bigr)^{-1}(x)$. 
    Then we have $y \in Y^{n_{\epsilon} + n_{F}} \subseteq X^{n_{F}} \subseteq B_{d}(y_{-}, \epsilon) \cap X^0_{\colour'}$.
    Thus\[
        v_{\colour'}(y) \leqslant v_{\colour'}(y_{-}) + \modufun(\epsilon) = \widetilde{v}(\widetilde{y}_{-}) + \modufun(\epsilon) < \delta_{1} / 2 \leqslant \normcontinuous{\widetilde{v}}{\splitsphere} - \delta_{1} / 2.
    \]

    Denote $N \define n_{\epsilon} + n_{F}$, which depends only on $F$, $\mathcal{C}$, $d$, $\modufun$, and $\delta_{1}$. 
    Write $ x_{X^{N}} \define \bigl( F^{N}|_{X^N} \bigr)^{-1}(x) $ for $\widetilde{\colour} \in \colours$ and $X^N \in \ccFTile{N}{\colour}{\widetilde{\colour}}$.
    By Definition~\ref{def:normalized split ruelle operator}, \eqref{eq:def:twisted partial Ruelle operator}, and Lemma~\ref{lem:norm of normalized split operator}, we have
    \begin{align*}
        \twistsplopt^{N}(\widetilde{v})(\widetilde{x}) 
        &= \toperator{N}{\colour}{\black}(v_{\black})(x) + \toperator{N}{\colour}{\white}(v_{\white})(x) \\
        &= v_{\colour'}(y) \myexp[\big]{ S_{N}^{F}\normpotential(y) + \log u_{\colour'}(y) - \log u_{\colour}(x) }    \\
        &\quad\ + \sum_{\widetilde{\colour} \in \colours}  \sum_{ X^N \in \ccFTile{N}{\colour}{\widetilde{\colour}} \setminus \{ Y^{N} \} } 
        v_{\widetilde{\colour}}( x_{X^{N}} ) \myexp[\big]{ S_{N}^{F}\normpotential( x_{X^{N}} ) + \log u_{\widetilde{\colour}}( x_{X^{N}} ) - \log u_{\colour}(x) }     \\
        &\leqslant \bigl( \normcontinuous{\widetilde{v}}{\splitsphere} - \delta_{1} / 2 \bigr) \myexp[\big]{ S_{N}^{F}\normpotential(y) + \log u_{\colour'}(y) - \log u_{\colour}(x) } \\
        &\quad\ + \normcontinuous{\widetilde{v}}{\splitsphere} \sum_{\widetilde{\colour} \in \colours}  \sum_{ X^N \in \ccFTile{N}{\colour}{\widetilde{\colour}} \setminus \{ Y^{N} \} }  \myexp[\big]{ S_{N}^{F}\normpotential( x_{X^{N}} ) + \log u_{\widetilde{\colour}}( x_{X^{N}} ) - \log u_{\colour}(x) }   \\
        &\leqslant \normcontinuous{\widetilde{v}}{\splitsphere}  \sum_{\widetilde{\colour} \in \colours} \, \sum_{ X^N \in \ccFTile{N}{\colour}{\widetilde{\colour}} }  \myexp[\big]{ S_{N}^{F}\normpotential( x_{X^{N}} ) + \log u_{\widetilde{\colour}}( x_{X^{N}} ) - \log u_{\colour}(x) } \\
        &\quad\ - 2^{-1} \delta_{1} \myexp[\big]{ S_{N}^{F}\normpotential(y) + \log u_{\colour'}(y) - \log u_{\colour}(x) } \\
        &= \normcontinuous{\widetilde{v}}{\splitsphere} - 2^{-1} \delta_{1} \myexp[\big]{ S_{N}^{F}\normpotential(y) + \log u_{\colour'}(y) - \log u_{\colour}(x) }.
        % \twistsplopt^{N}(\widetilde{v})(\widetilde{x}) 
        % &= \toperator{N}{\colour}{\black}(v_{\black})(x) + \toperator{N}{\colour}{\white}(v_{\white})(x) \\
        % &= v_{\colour'}(y) \myexp[\big]{ S_{N}^{F}\normpotential(y) + \log u_{\colour'}(y) - \log u_{\colour}(x) } \\
        % &\quad\ + \sum_{ \substack{ w = (F^{N}|_{X^N})^{-1}(x) \\ X^N \in \ccFTile{N}{\colour}{\colour'} \setminus \{ Y^{N} \} }} 
        % v_{\colour'}(w) \myexp[\big]{ S_{N}^{F}\normpotential(w) + \log u_{\colour'}(w) - \log u_{\colour}(x) } \\
        % &\quad\ + \sum_{ \substack{ w = (F^{N}|_{X^N})^{-1}(x) \\ X^N \in \ccFTile{N}{\colour}{\widetilde{\colour}} } } 
        % v_{\widetilde{\colour}}(w) \myexp[\big]{ S_{N}^{F}\normpotential(w) + \log u_{\widetilde{\colour}}(w) - \log u_{\colour}(x) } \\
        % &\leqslant \Bigl( \normcontinuous{\widetilde{v}}{\splitsphere} - \frac{\delta_{1}}{2} \Bigr) \myexp[\big]{ S_{N}^{F}\normpotential(y) + \log u_{\colour'}(y) - \log u_{\colour}(x) } \\
        % &\quad\ + \normcontinuous{\widetilde{v}}{\splitsphere} \!\!\! \sum_{ \substack{ w = (F^{N}|_{X^N})^{-1}(x) \\ X^N \in \ccFTile{N}{\colour}{\colour'} \setminus \{ Y^{N} \} }}  \myexp[\big]{ S_{N}^{F}\normpotential(w) + \log u_{\colour'}(w) - \log u_{\colour}(x) } \\
        % &\quad\ + \normcontinuous{\widetilde{v}}{\splitsphere} \! \sum_{ \substack{ w = (F^{N}|_{X^N})^{-1}(x) \\ X^N \in \ccFTile{N}{\colour}{\widetilde{\colour}} } } \myexp[\big]{ S_{N}^{F}\normpotential(w) + \log u_{\widetilde{\colour}}(w) - \log u_{\colour}(x) } \\
        % &\leqslant \normcontinuous{\widetilde{v}}{\splitsphere}  \sum_{\widetilde{\colour} \in \colours} \,  \sum_{ \substack{ w = (F^{N}|_{X^N})^{-1}(x) \\ X^N \in \ccFTile{N}{\colour}{\widetilde{\colour}} } } \myexp[\big]{ S_{N}^{F}\normpotential(w) + \log u_{\widetilde{\colour}}(w) - \log u_{\colour}(x) } \\
        % &\quad\ - \frac{\delta_{1}}{2} \myexp[\big]{ S_{N}^{F}\normpotential(y) + \log u_{\colour'}(y) - \log u_{\colour}(x) } \\
        % &= \normcontinuous{\widetilde{v}}{\splitsphere} - \frac{\delta_{1}}{2} \myexp[\big]{ S_{N}^{F}\normpotential(y) + \log u_{\colour'}(y) - \log u_{\colour}(x) }.        
    \end{align*}
    Similarly, there exists $z \define \bigl(F^{N}|_{Z^{N}}\bigr)^{-1}(x)$ for some $Z^N \in \ccFTile{N}{\colour}{\colour''}$ such that $z \in Z^{N} \subseteq B_{d}(y_{+}, \epsilon) \cap X^0_{\colour''}$ and 
    \[
        \twistsplopt^{N}(\widetilde{v})(\widetilde{x}) \geqslant -\normcontinuous{\widetilde{v}}{\splitsphere} + 2^{-1} \delta_{1} \myexp[\big]{ S_{N}^{F}\normpotential(z) + \log u_{\colour''}(z) - \log u_{\colour}(x) }.
    \]
    Recall that $\eigfun = \splfun \in \splfunspace$ is a continuous function on $\splitsphere$ given by Theorem~\ref{thm:existence of f invariant Gibbs measure}. 
    Then by \eqref{eq:two sides bounds for eigenfunction} in Theorem~\ref{thm:existence of f invariant Gibbs measure} we have\[
        \Csplratio^{-1} \leqslant \eigfun(\widetilde{w}) \leqslant \Csplratio, \qquad \text{for each } \widetilde{w} \in \splitsphere,
    \]
    where $\Csplratio \geqslant 1$ is the constant defined in \eqref{eq:const:Csplratio} in Lemma~\ref{lem:distortion lemma for subsystem}~\ref{item:lem:distortion lemma for subsystem:uniform bound} and depends only on $F$, $\mathcal{C}$, $d$, $\phi$, and $\holderexp$.
    Hence we get 
    \begin{equation}    \label{eq:temp:upper bound for norm of normalized split ruelle operator}
        \begin{split}
            \normcontinuous[\big]{\twistsplopt^{N}(\widetilde{v})}{\splitsphere} 
            &\leqslant \normcontinuous{\widetilde{v}}{\splitsphere} 
            - 2^{-1} \delta_{1} \Csplratio^{-2} \inf_{w \in S^2} \myexp[\big]{ S_{N}^{F}\normpotential(w) } \\
            &\leqslant \normcontinuous{\widetilde{v}}{\splitsphere} 
            - 2^{-1} \delta_{1} \Csplratio^{-2} \myexp{ - N \uniformnorm{\normpotential} }.
        \end{split}
    \end{equation}

    Now we bound $\uniformnorm{\normpotential} = \uniformnorm{\potential - \pressure}$. 
    By the definition of \holder norm in Section~\ref{sec:Notation} and the hypothesis, $\uniformnorm{\potential} \leqslant \holdernorm{\potential}{S^2} \leqslant K$. Recall the definition of topological pressure as given in \eqref{eq:def:topological pressure} and the Variational Principle~\eqref{eq:Variational Principle for pressure} in Subsection~\ref{sub:thermodynamic formalism}. 
    Then by Theorem~\ref{thm:subsystem characterization of pressure}, \eqref{eq:def:measure-theoretic pressure}, and the fact that $\uniformnorm{\potential} \leqslant K$, we get\[
        - K \leqslant \pressure \leqslant P(f, \potential) \leqslant h_{\operatorname{top}}(f) + K.
    \]    
    Then $|\pressure| \leqslant K + h_{\operatorname{top}}(f) = K + \log(\deg{f})$ (see \cite[Corollary~17.2]{bonk2017expanding}). 
    Hence \[
        \uniformnorm{\normpotential} \leqslant \uniformnorm{\potential} + |\pressure| \leqslant 2K +  \log(\deg{f}).
    \]

    By \eqref{eq:const:Csplratio} and \eqref{eq:const:C_1}, quantitatively,
    \[
        \Csplratio = (\deg{f})^{n_{F}} \myexp[\bigg]{ C_0 \frac{ \holderseminorm{\potential}{S^2} }{1 - \Lambda^{-\holderexp}} (\diam{d}{S^{2}} )^{\holderexp} + 2n_{F} \uniformnorm{\phi} },
    \]
    where $C_0 > 1$ is the constant depending only on $f$, $\mathcal{C}$, and $d$ from Lemma~\ref{lem:basic_distortion}. 
    Let\[
        \Csplratio' \define (\deg{f})^{n_{F}} \myexp[\bigg]{ \frac{ C_0 K }{1 - \Lambda^{-\holderexp}} (\diam{d}{S^{2}} )^{\holderexp} + 2n_{F} K }.
    \]
    Then we have $\Csplratio \leqslant \Csplratio'$ for each $\potential \in \holderspacesphere$ with $\holdernorm{\potential}{S^{2}} \leq K$, and the constant $\Csplratio'$ only depends on $F$, $\mathcal{C}$, $d$, $K$, and $\holderexp$. 

    Therefore, by \eqref{eq:temp:upper bound for norm of normalized split ruelle operator}, $\normcontinuous[\big]{\twistsplopt^{n}(\widetilde{v})}{\splitsphere} \leqslant \normcontinuous{\widetilde{v}}{\splitsphere} - \delta_2$, where\[
        \delta_{2} \define \frac{\delta_{1}}{2} \bigl( \Csplratio' \bigl)^{-2} \myexp{ - 2NK - N \log(\deg{f}) },
    \]
    which depends only on $F$, $\mathcal{C}$, $d$, $\modufun$, $\holderexp$, $K$, and $\delta_{1}$. 
    
    \smallskip

    Finally we show that $\spleigmea \bigl(\widetilde{\limitset} \bigr) = 1$.
    Indeed, by Proposition~\ref{prop:subsystem:properties invariant Jordan curve}~\ref{item:subsystem:properties invariant Jordan curve:decreasing relation of domains} and \eqref{eq:def:split tile of subsystem}, $\bigl\{ \bigcup\splDomain{n} \bigr\}_{n \in \n}$ is a decreasing sequence of sets. Then $\spleigmea\bigl(\spllimitset\bigr) = \lim\limits_{n \to +\infty} \spleigmea\bigl(\bigcup\splDomain{n}\bigr)$. Noting that $F$ is surjective since $F$ is strongly primitive, we have $\bigcup\splDomain{0} = \splitsphere$.
    Thus it suffices to show that
    \begin{equation}    \label{eq:temp:split eigenmeasure is the same on n tile}
        \spleigmea\Bigl( \bigcup\splDomain{n} \Bigr) = \spleigmea\Bigl( \bigcup\splDomain{n - 1} \Bigr)
    \end{equation}
    for each $n \in \n$. 
    
    For convenience we set $\spllimitset^{n} \define \bigcup\splDomain{n} \subseteq \splitsphere$ and $\limitset^{n}_{\colour} \define i_{\colour}^{-1}\bigl( \bigcup \splDomain{n} \bigr) \subseteq X^0_{\colour}$ for each $n \in \n_0$ and each $\colour \in \colours$. 
    Note that $\spllimitset^{n} = \limitset^{n}_{\black} \sqcup \limitset^{n}_{\white}$ and $\limitset^{n}_{\colour} = \bigcup \{ X^{n} \in \Domain{n} \describe X^{n} \subseteq X^{0}_{\colour} \}$ for each $n \in \n_{0}$ and each $\colour \in \colours$. 
    Let $n \in \n$ be arbitrary. By Proposition~\ref{prop:dual split operator}~\ref{item:prop:dual split operator:act on bound function} and \eqref{eq:Riesz representation}, we have
    \begin{align*}
        \bigl( \dualsplopt \bigr)^{n} \spleigmea\bigl( \spllimitset^{n-1} \bigr) 
        &= \bigl( \dualsplopt \bigr)^{n} \spleigmea\bigl( \limitset^{n-1}_{\black}, \limitset^{n-1}_{\white} \bigr) 
        = \bigl\langle \spleigmea, \splopt^n \bigl(\mathbbm{1}_{\limitset^{n-1}_{\black}}, \mathbbm{1}_{\limitset^{n-1}_{\white}} \bigr) \bigr\rangle \\
        &=  \bigl\langle m_{\black},  \pi_{\black} \bigl(\splopt^n \bigl(\mathbbm{1}_{\limitset^{n-1}_{\black}}, \mathbbm{1}_{\limitset^{n-1}_{\white}} \bigr) \bigr)  \bigr\rangle
        +  \bigl\langle m_{\white},  \pi_{\white} \bigl( \splopt^n \bigl(\mathbbm{1}_{\limitset^{n-1}_{\black}}, \mathbbm{1}_{\limitset^{n-1}_{\white}}\bigr) \bigr)  \bigr\rangle , \\
        \bigl( \dualsplopt \bigr)^{n} \spleigmea\bigl( \spllimitset^{n} \bigr) %%%%%%%%
        &= \bigl( \dualsplopt \bigr)^{n} \spleigmea\bigl( \limitset^{n}_{\black}, \limitset^{n}_{\white} \bigr) 
        = \bigl\langle \spleigmea, \splopt^n \bigl(\mathbbm{1}_{\limitset^{n}_{\black}}, \mathbbm{1}_{\limitset^{n}_{\white}} \bigr) \bigr\rangle \\
        &=  \bigl\langle m_{\black},  \pi_{\black} \bigl(\splopt^n \bigl(\mathbbm{1}_{\limitset^{n}_{\black}}, \mathbbm{1}_{\limitset^{n}_{\white}} \bigr) \bigr)  \bigr\rangle
        +  \bigl\langle m_{\white},  \pi_{\white} \bigl( \splopt^n \bigl(\mathbbm{1}_{\limitset^{n}_{\black}}, \mathbbm{1}_{\limitset^{n}_{\white}}\bigr) \bigr)  \bigr\rangle.
    \end{align*}
    Since $\dualsplopt\spleigmea = \eigenvalue \spleigmea$, it suffices to show that\[
        \pi_{\colour} \bigl( \splopt^n \bigl(\mathbbm{1}_{\limitset^{n-1}_{\black}}, \mathbbm{1}_{\limitset^{n-1}_{\white}} \bigr) \bigr) 
        = \pi_{\colour} \bigl( \splopt^n \bigl( \mathbbm{1}_{\limitset^{n}_{\black}}, \mathbbm{1}_{\limitset^{n}_{\white}} \bigr) \bigr)
    \]
    for each $\colour \in \colours$. 
    Indeed, by \eqref{eq:projection on product function spaces}, \eqref{eq:iteration of split-partial ruelle operator}, and \eqref{eq:definition of partial Ruelle operators},
    \begin{align*}
        \pi_{\colour} \bigl( \splopt^n \bigl(\mathbbm{1}_{\limitset^{n-1}_{\black}}, \mathbbm{1}_{\limitset^{n-1}_{\white}} \bigr) \bigr) 
        &= \paroperator{n}{\colour}{\black} \bigl(\mathbbm{1}_{\limitset^{n-1}_{\black}} \bigr) + \paroperator{n}{\colour}{\white} \bigl(\mathbbm{1}_{\limitset^{n-1}_{\white}}\bigr) \\
        &= \sum_{\colour' \in \colours} \sum_{ X^n \in \ccFTile{n}{\colour}{\colour'} }   \bigl( \mathbbm{1}_{ \limitset^{n-1}_{\colour'} } \!\cdot \myexp[\big]{ S_{n}^{F}\phi } \bigr) \circ (F|_{X^n})^{-1}   \\
        &= \sum_{\colour' \in \colours} \sum_{ X^n \in \ccFTile{n}{\colour}{\colour'} }   \bigl(\mathbbm{1}_{ \limitset^{n}_{\colour'} } \!\cdot \myexp[\big]{ S_{n}^{F}\phi } \bigr) \circ (F|_{X^n})^{-1}   \\
        &= \pi_{\colour} \bigl( \splopt^n \bigl( \mathbbm{1}_{\limitset^{n}_{\black}}, \mathbbm{1}_{\limitset^{n}_{\white}} \bigr) \bigr),
    \end{align*}
    where the third equality holds since $X^n \subseteq \limitset^{n}_{\colour'} \subseteq \limitset^{n-1}_{\colour'}$ for each $\colour' \in \colours$ and each $X^n \in \ccFTile{n}{\colour}{\colour'}$. Thus \eqref{eq:temp:split eigenmeasure is the same on n tile} holds and we deduce that $\spleigmea \bigl(\widetilde{\limitset} \bigr) = 1$.
\end{proof}


\begin{theorem}    \label{thm:converge of uniform norm of normalized split ruelle operator}
    Let $f$, $\mathcal{C}$, $F$, $d$, $\Lambda$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive.
    Let $\moduconst \in (0, +\infty)$ be a constant and $\modufun \colon [0, +\infty) \mapping [0, +\infty)$ an abstract modulus of continuity. 
    Let $H$ be a bounded subset of $\holderspacesphere$ for some $\holderexp \in (0, 1]$.
    Then for each $\widetilde{v} \in \splmoduspace$, each $\potential \in H$, and each choice of $\spleigmea \in \probmea{\splitsphere}$ from Theorem~\ref{thm:subsystem:eigenmeasure existence and basic properties}, we have
    \begin{equation}    \label{eq:converge of uniform norm of normed split ruelle operator}
         \lim_{n \to +\infty} \normcontinuous[\bigg]{\normsplopt^{n}(\widetilde{v}) - \eigfun \int \! \widetilde{v} \,\mathrm{d}\spleigmea}{\splitsphere} = 0.
    \end{equation}
    If, in addition, $\int \! \widetilde{v} \eigfun \,\mathrm{d}\spleigmea = 0$, then
    \begin{equation}    \label{eq:converge of uniform norm of normalized split ruelle operator}
        \lim_{n \to +\infty} \normcontinuous[\big]{\twistsplopt^{n}(\widetilde{v})}{\splitsphere} = 0.
    \end{equation}
    Moreover, the convergence in both \eqref{eq:converge of uniform norm of normed split ruelle operator} and \eqref{eq:converge of uniform norm of normalized split ruelle operator} is uniform in $\widetilde{v} \in \splmoduspace$, $\potential \in H$, and the choice of $\spleigmea$.
\end{theorem}
% \begin{rmk}
%     The equation~\eqref{eq:converge of uniform norm of normalized split ruelle operator} demonstrates the contracting behavior of $\twistsplopt$ on a codimension-$1$ subspace of $C(\splitsphere)$.
% \end{rmk}
\begin{proof}
    Fix a constant $K \in [0, +\infty)$ such that $\holdernorm{\potential}{S^2} \leqslant K$ for each $\potential \in H$. 
    Let $\mathcal{M}_{F, \potential}$ be the set of possible choices of $\spleigmea \in \probmea{\splitsphere}$ from Theorem~\ref{thm:subsystem:eigenmeasure existence and basic properties}, i.e., 
    \begin{equation}    \label{eq:temp:set of eigenmeasure}
        \mathcal{M}_{F, \potential} \define \bigl\{ \splmeav \in \probmea{\splitsphere} \describe \dualsplopt\splmeav = \eigenvalue \splmeav \text{ for some } c \in \real \bigr\}.
    \end{equation}

    We recall that $\splmea \in \probmea{\splitsphere}$ defined in Theorem~\ref{thm:existence of f invariant Gibbs measure} by $\splmea = \eigfun \spleigmea$ depends on the choice of $\spleigmea$.

    Define for each $n \in \n_0$,\[
        a_n \define \sup \Bigl\{ \normcontinuous[\big]{\twistsplopt^{n}(\widetilde{v})}{\splitsphere} \describe \potential \in H, \, \widetilde{v} \in \splmoduspace, \, \int \! \widetilde{v} \eigfun \,\mathrm{d}\spleigmea = 0, \, \spleigmea \in \mathcal{M}_{F, \potential} \Bigr\}.
    \]
    By Lemma~\ref{lem:norm of normalized split operator}, $\normcontinuous[\big]{\twistsplopt}{\splitsphere} = 1$, so $\normcontinuous[\big]{\twistsplopt^{n}(\widetilde{v})}{\splitsphere}$ is non-increasing in $n$ for fixed $\potential \in H$ and $\widetilde{v} \in \splmoduspace$. Note that $a_0 \leqslant \moduconst < +\infty$. Thus $\{a_{n}\}_{n \in \n_0}$ is a non-increasing sequence of non-negative real numbers.

    Suppose now that $\lim_{n \to +\infty} a_{n} = a > 0$. By Proposition~\ref{prop:modulus for function under split ruelle operator}, there exists an abstract modulus of continuity $\widetilde{\modufun}$ such that \[
        \Bigl\{ \twistsplopt^{n}(\widetilde{v}) \describe n \in \n_0, \, \potential \in H, \, \widetilde{v} \in \splmoduspace \Bigr\} \subseteq \splmoduspace[\moduconst][\widetilde{\modufun}].
    \]
    Note that for each $\potential \in H$, each $n \in \n_0$, and each $\widetilde{v} \in \splmoduspace$ with $\int \! \widetilde{v}\eigfun \,\mathrm{d}\spleigmea = 0$, it follows from \eqref{eq:equilibrium state is eigenmeasure of dual normalized split operator} that \[
        \int \! \twistsplopt^{n}(\widetilde{v}) \eigfun \,\mathrm{d}\spleigmea = \int \! \twistsplopt^{n}(\widetilde{v}) \,\mathrm{d}\splmea = \int \! \widetilde{v} \,\mathrm{d}\splmea = 0.
    \] 
    Then by applying Lemma~\ref{lem:upper bound for uniform norm of normalized split ruelle operator} with $\widetilde{\modufun}$, $\holderexp$, $K$, and $\delta_{1} = a/2$, we find constants $n_0 \in \n$ and $\delta_{2} > 0$ such that \[
        \normcontinuous[\big]{\twistsplopt^{n_{0}}\bigl( \twistsplopt^{n}(\widetilde{v}) \bigl)  }{\splitsphere} 
        \leqslant \normcontinuous[\big]{\twistsplopt^{n}(\widetilde{v})}{\splitsphere} - \delta_{2},
    \]  
    for each $n \in \n_0$, each $\potential \in H$, each $\spleigmea \in \mathcal{M}_{F, \potential}$, and each $\widetilde{v} \in \splmoduspace$ with $\int \! \widetilde{v} \eigfun \,\mathrm{d}\spleigmea = 0$ and $\normcontinuous[\big]{\twistsplopt^{n}(\widetilde{v})}{\splitsphere} \geqslant a/2$. Since $\lim_{n \to +\infty} a_{n} = a$, we can fix integer $m > 1$ sufficiently large such that $a_{m} \leqslant a + \delta_{2}/2$. 
    Then for each $\potential \in H$, each $\spleigmea \in \mathcal{M}_{F, \potential}$, and each $\widetilde{v} \in \splmoduspace$ with $\int \! \widetilde{v} \eigfun \,\mathrm{d}\spleigmea = 0$ and $\normcontinuous[\big]{\twistsplopt^{m}(\widetilde{v})}{\splitsphere} \geqslant a/2$. we have\[
        \normcontinuous[\big]{\twistsplopt^{n_{0} + m}(\widetilde{v})}{\splitsphere} 
        \leqslant \normcontinuous[\big]{\twistsplopt^{m}(\widetilde{v})}{\splitsphere} - \delta_{2} 
        \leqslant a_{m} - \delta_{2} \leqslant a - \delta_{2}/2.
    \]
    On the other hand, since $\normcontinuous[\big]{\twistsplopt^{n}(\widetilde{v})}{\splitsphere}$ is non-increasing in $n$, we have that for each $\potential \in H$, each $\spleigmea \in \mathcal{M}_{F, \potential}$, and each $\widetilde{v} \in \splmoduspace$ with $\int \! \widetilde{v} \eigfun \,\mathrm{d}\spleigmea = 0$ and $\normcontinuous[\big]{\twistsplopt^{m}(\widetilde{v})}{\spllimitset} < a/2$, the following holds: \[
        \normcontinuous[\big]{\twistsplopt^{n_{0} + m}(\widetilde{v})}{\splitsphere} 
        \leqslant \normcontinuous[\big]{\twistsplopt^{m}(\widetilde{v})}{\splitsphere} < a/2.
    \]
    Thus $a_{n_{0} + m} \leqslant \max \bigl\{ a - \delta_{2}/2, \, a/2 \bigr\} < a$, contradicting the fact that $\{a_{n}\}_{n \in \n_0}$ is a non-increasing sequence and the assumption that $\lim_{n \to +\infty} a_{n} = a$. This proves the uniform convergence in \eqref{eq:converge of uniform norm of normalized split ruelle operator}.

    Next, we prove the uniform convergence in \eqref{eq:converge of uniform norm of normed split ruelle operator}. By Lemma~\ref{lem:norm of normalized split operator} and \eqref{eq:iteration of normalized split ruelle operator} in Lemma~\ref{lem:iteration of normalized split ruelle operator}, for each $\widetilde{v} \in \splmoduspace$, each $\potential \in H$, and each $\spleigmea \in \mathcal{M}_{F, \potential}$, we have
    \begin{equation}    \label{eq:temp:upper bound for norm associated with normed split ruelle operator}
        \begin{split}
            \normcontinuous[\bigg]{\normsplopt^{n}(\widetilde{v}) - \eigfun \int \! \widetilde{v} \,\mathrm{d}\spleigmea}{\splitsphere} 
            &\leqslant \normcontinuous{\eigfun}{\splitsphere} \normcontinuous[\bigg]{ \frac{1}{\eigfun} \normsplopt^{n}(\widetilde{v}) - \int \! \widetilde{v} \,\mathrm{d}\spleigmea}{\splitsphere} \\
            &= \normcontinuous{\eigfun}{\splitsphere} \normcontinuous[\bigg]{ \twistsplopt^{n}\biggl( \frac{\widetilde{v}}{\eigfun} \biggr) - \int \! \frac{\widetilde{v}}{\eigfun} \,\mathrm{d}\splmea}{\splitsphere} \\
            &= \normcontinuous{\eigfun}{\splitsphere} \normcontinuous[\bigg]{ \twistsplopt^{n}\biggl( \frac{\widetilde{v}}{\eigfun} - \indicator{\splitsphere} \int \! \frac{\widetilde{v}}{\eigfun} \,\mathrm{d}\splmea \biggr) }{\splitsphere}.
        \end{split}
    \end{equation}
    By \eqref{eq:eigenfunction of normed split operator} in Theorem~\ref{thm:existence of f invariant Gibbs measure}, we have
    \begin{equation}    \label{eq:temp:bounds for norm of eigenfunction}
        \Csplratio^{-1} \leqslant \normcontinuous{\eigfun}{\splitsphere} \leqslant \Csplratio,
    \end{equation}
    where $\Csplratio \geqslant 1$ is the constant defined in \eqref{eq:const:Csplratio} in Lemma~\ref{lem:distortion lemma for subsystem}~\ref{item:lem:distortion lemma for subsystem:uniform bound} and depends only on $F$, $\mathcal{C}$, $d$, $\phi$, and $\holderexp$.
    By \eqref{eq:const:Csplratio} and \eqref{eq:const:C_1}, quantitatively,
    \[
        \Csplratio = (\deg{f})^{n_{F}} \myexp[\bigg]{ C_0 \frac{ \holderseminorm{\potential}{S^2} }{1 - \Lambda^{-\holderexp}} (\diam{d}{S^{2}} )^{\holderexp} + 2n_{F} \uniformnorm{\phi} },
    \]
    where $C_0 > 1$ is the constant depending only on $f$, $\mathcal{C}$, and $d$ from Lemma~\ref{lem:basic_distortion} and $n_{F} \in \n$ is the constant depending only on $F$ and $\mathcal{C}$ from Definition~\ref{def:primitivity of subsystem} since $F$ is primitive. 
    Let\[
        \Csplratio' \define (\deg{f})^{n_{F}} \myexp[\bigg]{ \frac{ C_0 K }{1 - \Lambda^{-\holderexp}} (\diam{d}{S^{2}} )^{\holderexp} + 2n_{F} K }.
    \]
    Then we have $\Csplratio \leqslant \Csplratio'$ for each $\potential \in \holderspacesphere$ with $\holdernorm{\potential}{S^{2}} \leq K$, and the constant $\Csplratio'$ only depends on $F$, $\mathcal{C}$, $d$, $K$, and $\holderexp$. 
    Let \[
        \widetilde{w} \define \frac{\widetilde{v}}{\eigfun} - \indicator{\splitsphere} \int \! \frac{\widetilde{v}}{\eigfun} \,\mathrm{d}\splmea \in C(\splitsphere).
    \] 
    Then $\normcontinuous{\widetilde{w}}{\splitsphere} \leqslant 2 \normcontinuous{ \widetilde{v} / \eigfun} {\splitsphere} \leqslant 2 \moduconst \Csplratio'$.
    Due to the first inequality in \eqref{eq:two sides bounds for eigenfunction} and the fact that $\eigfun \in \splholderspace$ by Theorem~\ref{thm:existence of f invariant Gibbs measure}, we can apply Lemma~\ref{lem:product and inverse of modulus of continuity} and conclude that there exists an abstract modulus of continuity $\widehat{\modufun}$ associated with $\frac{\widetilde{v}}{\eigfun}$ such that $\widehat{\modufun}$ is independent of the choices of $\widetilde{v} \in \splmoduspace$, $\potential \in H$, and $\spleigmea \in \mathcal{M}_{F, \potential}$. 
    Thus $\widetilde{w} \in \moduspace[\widehat{\moduconst}][\widehat{\modufun}]$, where $\widehat{\moduconst} \define 2 \moduconst \Csplratio'$. Note that $\int \! \widetilde{w} \eigfun \,\mathrm{d}\spleigmea = \int \! \widetilde{w} \,\mathrm{d}\splmea = 0$. Finally, we can apply the uniform convergence in \eqref{eq:converge of uniform norm of normalized split ruelle operator} with $\widetilde{v} = \widetilde{w}$  to conclude the uniform convergence in \eqref{eq:converge of uniform norm of normed split ruelle operator} by \eqref{eq:temp:upper bound for norm associated with normed split ruelle operator} and \eqref{eq:temp:bounds for norm of eigenfunction}.   
\end{proof}


The following proposition is an immediate consequence of Theorem~\ref{thm:converge of uniform norm of normalized split ruelle operator}.
\begin{proposition}    \label{prop:convergence to equilibrium state under dual split Ruelle operator}
    Let $f$, $\mathcal{C}$, $F$, $d$, $\potential$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive.
    Let $\splmea \in \probmea{\splitsphere}$ be a Borel probability measure defined in Theorem~\ref{thm:existence of f invariant Gibbs measure}. 
    Then for each Borel probability measure $\splmeav \in \probmea{\splitsphere}$, we have
    \[
        \bigl( \dualtwistsplopt \bigl)^{n}\splmeav \weakconverge \splmea \quad \text{ as } n \to +\infty.
    \]
\end{proposition}
\begin{proof}
    Recall that for each $\widetilde{v} \in C(\splitsphere)$, there exists some abstract modulus of continuity $\modufun$ such that $\widetilde{v} \in \moduspace[][][S^2]$, where $\moduconst \define \normcontinuous{\widetilde{v}}{\splitsphere}$. 
    Recall from Theorem~\ref{thm:existence of f invariant Gibbs measure} that $\splmea = \eigfun \spleigmea$. 
    Then by Lemma~\ref{lem:norm of normalized split operator} and \eqref{eq:converge of uniform norm of normalized split ruelle operator} in Theorem~\ref{thm:converge of uniform norm of normalized split ruelle operator},
    \[
        \begin{split}
            &\quad\, \lim_{n \to +\infty} \functional[\big]{ \bigl( \dualtwistsplopt \bigl)^{n}\splmeav }{\widetilde{v}} \\
            &= \lim_{n \to +\infty} \bigl(  \functional[\big]{ \splmeav }{ \twistsplopt^{n}\bigl( \widetilde{v} - \functional{\splmea}{\widetilde{v}}\indicator{\splitsphere} \bigl) } 
                + \functional[\big]{\splmeav}{ \twistsplopt^{n} \bigl( \functional{\splmea}{\widetilde{v}} \indicator{\splitsphere} \bigl) }  \bigl)\\
            &= 0 + \functional[\big]{\splmeav}{ \functional{\splmea}{\widetilde{v}} \indicator{\splitsphere} } = \functional{\splmeav}{\widetilde{v}},
        \end{split}
    \]
    for each $\widetilde{v} \in C(\splitsphere)$. 
    This completes the proof.
\end{proof}

We now verity the spectral gap for $\twistsplopt$.

% \begin{theorem}    \label{thm:exponential decay of uniform norm of normalized split ruelle operator}
%     Let $f$, $\mathcal{C}$, $F$, $d$, $\potential$, $\holderexp$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$.
%     Let $F \in \subsystem$ be strongly primitive.
% \end{theorem}











\subsection{Uniqueness}%
\label{sub:Uniqueness}
In this subsection we prove Theorem~\ref{thm:subsystem:uniqueness of equilibrium state}. 

\smallskip

Theorem~\ref{thm:converge of uniform norm of normalized split ruelle operator} implies in particular the uniqueness of $\spleigmea \in \probmea{\splitsphere}$ defined in Theorem~\ref{thm:subsystem:eigenmeasure existence and basic properties}.

\begin{proposition}    \label{prop:uniqueness of eigenmeasure subsystem}
    Let $f$, $\mathcal{C}$, $F$, $d$, $\potential$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive.
    Then the measure $\eigmea = \spleigmea \in \probmea{\splitsphere}$ defined in Theorem~\ref{thm:subsystem:eigenmeasure existence and basic properties} is unique, i.e., $\spleigmea$ is the unique Borel probability measure on $\splitsphere$ that satisfies $\dualsplopt\spleigmea = \eigenvalue \spleigmea$ for some constant $\eigenvalue \in \real$. 
    Moreover, the measure $\equstate = \splmea \define \eigfun \spleigmea$ from Theorem~\ref{thm:existence of f invariant Gibbs measure} is the unique Borel probability measure on $\splitsphere$ that satisfies $\dualtwistsplopt\splmea = \splmea$.
\end{proposition}
Note that by Theorem~\ref{thm:existence of equilibrium state for subsystem}, $\equstate$ is an equilibrium state for $\limitmap$ and $\potential$.
\begin{proof}
    Let $\spleigmea, \, \spleigmeaanother \in \probmea{\splitsphere}$ be two measures, both of which arise from Theorem~\ref{thm:subsystem:eigenmeasure existence and basic properties}. Note that for each $\widetilde{v} = \splfunv \in C(\splitsphere)$, there exists some abstract modulus of continuity $\modufun$ such that $\widetilde{v} = \splfunv \in \splmoduspace$, where $\moduconst \define \normcontinuous{\widetilde{v}}{\splitsphere}$.
    Then by \eqref{eq:converge of uniform norm of normed split ruelle operator} in Theorem~\ref{thm:converge of uniform norm of normalized split ruelle operator} and \eqref{eq:two sides bounds for eigenfunction} in Theorem~\ref{thm:existence of f invariant Gibbs measure}, we see that $\int \! \widetilde{v} \,\mathrm{d}\spleigmea = \int \! \widetilde{v} \,\mathrm{d}\spleigmeaanother$ for each $\widetilde{v} \in C(\splitsphere)$. Thus $\spleigmea = \spleigmeaanother$.

    Recall from \eqref{eq:equilibrium state is eigenmeasure of dual normalized split operator} that $\dualtwistsplopt\splmea = \splmea$. Suppose $\splmeav \in \probmea{\splitsphere}$ is another measure with $\dualtwistsplopt\splmeav = \splmeav$. 
    Note that by \eqref{eq:two sides bounds for eigenfunction} in Theorem~\ref{thm:existence of f invariant Gibbs measure}, there exists a constant $C > 0$ such that $\eigfun(\widetilde{x}) \geqslant C$ for each $\widetilde{x}$. 
    Then by \eqref{eq:def:normalized split Ruelle operator} in Definition~\ref{def:normalized split ruelle operator}, for each $\widetilde{v} \in C(\splitsphere)$, we have
    \[
        \begin{split}
            \functional[\Big]{\dualtwistsplopt\splmeav}{\widetilde{v}} &= \functional[\Big]{\splmeav}{\twistsplopt(\widetilde{v})} = \functional[\Big]{\splmeav}{ \frac{1}{\eigfun}  \normsplopt( \eigfun \widetilde{v})} \\
            &= \functional[\bigg]{ \frac{\splmeav}{\eigfun} }{\normsplopt(\eigfun \widetilde{v})} = \functional[\bigg]{\eigfun \normdualsplopt\biggl(\frac{\splmeav}{\eigfun}\biggr)}{\widetilde{v}}.
        \end{split}
    \]
    Thus $\eigfun \normdualsplopt\Bigl(\frac{\splmeav}{\eigfun}\Bigr) = \dualtwistsplopt\splmeav = \splmeav$, i.e., $\normdualsplopt\Bigl(\frac{\splmeav}{\eigfun}\Bigr) = \frac{\splmeav}{\eigfun}$. 
    Denote $\lambda \define \functional[\Big]{\frac{\splmeav}{\eigfun}}{\indicator{\splitsphere}} > 0$. 
    Then by \eqref{eq:def:normed split operator} and Theorem~\ref{thm:subsystem characterization of pressure}, we have $\dualsplopt\Bigl(\frac{\splmeav}{\lambda \eigfun}\Bigr) = e^{\pressure} \frac{\splmeav}{\lambda \eigfun}$.
    Noting that $\frac{\splmeav}{\lambda \eigfun}$ is a Borel probability measure on $\splitsphere$, we conclude that $\frac{\splmeav}{\lambda \eigfun} = \spleigmea$. 
    Hence $\splmeav = \lambda \eigfun \spleigmea = \lambda \splmea$. 
    Since $\juxtapose{\splmeav}{\splmea} \in \probmea{\splitsphere}$, we get $\lambda = 1$ and $\splmeav = \splmea$. 
    Thus $\splmea$ is the only Borel probability measure on $\splitsphere$ that satisfies $\dualtwistsplopt\splmea = \splmea$.
\end{proof}


We follow the conventions discussed in Remarks~\ref{rem:disjoint union} and \ref{rem:probability measure in split setting}.
\begin{lemma}     \label{lem:converge of derivative for pressure of subsystem} \def\ncolour{\colour_{n}}
    Let $f$, $\mathcal{C}$, $F$, $d$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive.
    Let $\moduconst \geqslant 0$ be a constant and $\modufun$ an abstract modulus of continuity. 
    Let $H$ be a bounded subset of $\holderspacesphere$ for some $\holderexp \in (0, 1]$.
    Fix arbitrary sequence $\sequen{x_{n}}$ of points in $S^2$ and sequence $\sequen{\ncolour}$ of colors in $\colours$ that satisfies $x_{n} \in X^0_{\ncolour}$ for each $n \in \n$.
    Then for each $v \in \moduspace[\moduconst][\modufun][S^2]$ and each $\potential \in H$, we have
    \begin{equation}    \label{eq:converge of derivative for pressure of subsystem}
        \lim_{n \to +\infty}  \frac{ \frac{1}{n} \sum\limits_{ X^n \in \ccFTile{n}{\ncolour}{} } \bigl(S_{n}^{F}v( x_{X^{n}} )\bigr) \myexp[\big]{ S^{F}_{n} \phi ( x_{X^{n}} ) } }{ \sum\limits_{ X^n \in \ccFTile{n}{\ncolour}{} } \myexp[\big]{ S^{F}_{n} \phi ( x_{X^{n}} ) } }
        %= \int_{\blacktile} \! v_{\black} \,\mathrm{d}\equstate + \int_{\whitetile} \! v_{\white} \,\mathrm{d}\equstate 
        = \int_{S^2} \! v \,\mathrm{d}\equstate,
    \end{equation}
    where we denote $x_{X^{n}} \define (F^{n}|_{X^{n}})^{-1}(x_{n})$ for each $X^{n} \in \ccFTile{n}{\ncolour}{}$, and $\equstate \in \probsphere$ is defined in Theorem~\ref{thm:existence of f invariant Gibbs measure}. 
    Moreover, the convergence is uniform in $v \in \moduspace[\moduconst][\modufun][S^2]$ and $\potential \in H$.
\end{lemma}
\begin{proof}
    \def\ncolour{\colour_{n}}
    By Lemma~\ref{lem:iteration of split-partial ruelle operator} and Definition~\ref{def:partial Ruelle operator}, for each $n \in \n$, $v \in \moduspace[\moduconst][\modufun][S^2]$, and each $\potential \in H$,
    \begin{align*}
        \frac{ \frac{1}{n} \sum\limits_{ X^n \in \ccFTile{n}{\ncolour}{} } \bigl(S_{n}^{F}v( x_{X^{n}} )\bigr) \myexp[\big]{ S^{F}_{n} \phi ( x_{X^{n}} ) } }{ \sum\limits_{ X^n \in \ccFTile{n}{\ncolour}{} } \myexp[\big]{ S^{F}_{n} \phi ( x_{X^{n}} ) } }
        &= \frac{ \frac{1}{n} \sum\limits_{j=0}^{n-1} \sum\limits_{ X^n \in \ccFTile{n}{\ncolour}{} } v(f^{j}( x_{X^{n}} )) \myexp[\big]{ S^{F}_{n} \phi ( x_{X^{n}} ) } }{ \bigl( \splopt^{n}\bigl(\indicator{\splitsphere}\bigr) \bigr)(x_{n}, \ncolour) } \\
        &= \frac{ \frac{1}{n} \sum\limits_{j=0}^{n-1} \Bigl( \splopt^{n}(\widetilde{v\circ f^{j}}) \Bigl)(x_{n}, \ncolour) }{ \bigl( \splopt^{n}\bigl(\indicator{\splitsphere}\bigr) \bigr)(x_{n}, \ncolour) },
    \end{align*}
    where, by abuse of notation, for each $u \in C(S^2)$ we denote by $\widetilde{u}$ the continuous function on $\splitsphere$ given by $\widetilde{u}(\widetilde{z}) \define u(z)$ for each $\widetilde{z} = (z, \colour) \in \splitsphere$. 
    Note that by Lemma~\ref{lem:iteration of split-partial ruelle operator} and Definition~\ref{def:partial Ruelle operator}, for each $j \in \n_0$, 
    \[
        \splopt^{j}(\widetilde{v \circ f^{j}}) = \widetilde{v} \, \splopt^{j}\bigl(\indicator{\splitsphere}\bigr).
    \]
    Therefore, \[
        \begin{split}
        \frac{ \frac{1}{n} \sum\limits_{j=0}^{n-1} \Bigl( \splopt^{n}(\widetilde{v\circ f^{j}}) \Bigl)(x_{n}, \ncolour) }{ \bigl( \splopt^{n}\bigl(\indicator{\splitsphere}\bigr) \bigr)(x_{n}, \ncolour) } 
        &= \frac{ \frac{1}{n} \sum\limits_{j=0}^{n-1} \bigl( \splopt^{n - j} \bigl( \widetilde{v}\, \splopt^{j}\bigl(\indicator{\splitsphere}\bigr) \bigr) \bigl)(x_{n}, \ncolour) }{ \bigl( \splopt^{n}\bigl(\indicator{\splitsphere}\bigr) \bigr)(x_{n}, \ncolour) }  \\
        &= \frac{ \frac{1}{n} \sum\limits_{j=0}^{n-1} \bigl( \normsplopt^{n - j} \bigl( \widetilde{v}\, \normsplopt^{j}\bigl(\indicator{\splitsphere}\bigr) \bigr) \bigl)(x_{n}, \ncolour) }{ \bigl( \normsplopt^{n}\bigl(\indicator{\splitsphere}\bigr) \bigr)(x_{n}, \ncolour) }.
        \end{split}
    \]
    By Proposition~\ref{prop:modulus for function under split ruelle operator}, $\bigl\{ \normsplopt^{n}\bigl( \indicator{\splitsphere} \bigl) \describe n \in \n_0 \bigr\} \subseteq \splmoduspace[\widehat{\moduconst}][\widehat{\modufun}]$, for some constant $\widehat{\moduconst} \geqslant 0$ and some abstract modulus of continuity $\widehat{\modufun}$, which are independent of the choice of $\potential \in H$. Thus by Lemma~\ref{lem:product and inverse of modulus of continuity},
    \begin{equation}    \label{eq:temp:modulus of product of function and split operator}
        \bigl\{ \widetilde{v} \, \normsplopt^{n}\bigl( \indicator{\splitsphere} \bigl) \describe n \in \n_0, \, v \in \moduspace[][][S^2] \bigr\} \subseteq \splmoduspace[\moduconst_1][\modufun_1],
    \end{equation}
    for some constant $\moduconst_1 \geqslant 0$ and some abstract modulus of continuity $\modufun_1$, which are independent of the choice of $\potential \in H$.

    By Theorem~\ref{thm:converge of uniform norm of normalized split ruelle operator} and Proposition~\ref{prop:uniqueness of eigenmeasure subsystem}, we have
    \begin{equation}    \label{eq:temp:converge indicator under operator}
        \normcontinuous[\big]{ \normsplopt^{k}\bigl( \indicator{\splitsphere} \bigl) - \eigfun }{\splitsphere} \converge 0,
    \end{equation}
    as $k \to +\infty$, uniformly in $\potential \in H$. Moreover, by \eqref{eq:temp:modulus of product of function and split operator}, the independence of $\moduconst_1$ and $\modufun_1$ on $\potential \in H$ in \eqref{eq:temp:modulus of product of function and split operator}, Theorem~\ref{thm:converge of uniform norm of normalized split ruelle operator}, and Proposition~\ref{prop:uniqueness of eigenmeasure subsystem}, we have 
    \begin{equation}    \label{eq:temp:converge product function under operator}
           \normcontinuous[\bigg]{ \normsplopt^{k}\Bigl( \widetilde{v} \, \normsplopt^{j} \bigl( \indicator{\splitsphere} \bigr) \Bigl) - \eigfun \int \! \widetilde{v} \, \normsplopt^{j} \bigl( \indicator{\splitsphere} \bigr) \,\mathrm{d}\spleigmea }{\splitsphere} \converge 0,
    \end{equation}   
    as $k \to +\infty$, uniformly in $j \in \n_0$, $\potential \in H$, and $v \in \moduspace[][][S^2]$.

    Fix a constant $K \geqslant 0$ such that for each $\potential \in H$, $\holdernorm{\potential}{S^2} \leqslant K$.
    By \eqref{eq:eigenfunction of normed split operator} in Theorem~\ref{thm:existence of f invariant Gibbs measure}, we have
    \begin{equation}    \label{eq:temp:bounds for norm of eigenfunction use in converge}
        \Csplratio^{-1} \leqslant \normcontinuous{\eigfun}{\splitsphere} \leqslant \Csplratio,
    \end{equation}
    where $\Csplratio \geqslant 1$ is the constant defined in \eqref{eq:const:Csplratio} in Lemma~\ref{lem:distortion lemma for subsystem}~\ref{item:lem:distortion lemma for subsystem:uniform bound} and depends only on $F$, $\mathcal{C}$, $d$, $\phi$, and $\holderexp$.
    By \eqref{eq:const:Csplratio} and \eqref{eq:const:C_1}, quantitatively,
    \[
        \Csplratio = (\deg{f})^{n_{F}} \myexp[\bigg]{ C_0 \frac{ \holderseminorm{\potential}{S^2} }{1 - \Lambda^{-\holderexp}} (\diam{d}{S^{2}} )^{\holderexp} + 2n_{F} \uniformnorm{\phi} },
    \]
    where $C_0 > 1$ is the constant depending only on $f$, $\mathcal{C}$, and $d$ from Lemma~\ref{lem:basic_distortion} and $n_{F} \in \n$ is the constant depending only on $F$ and $\mathcal{C}$ from Definition~\ref{def:primitivity of subsystem} since $F$ is primitive. 
    Let\[
        \Csplratio' \define (\deg{f})^{n_{F}} \myexp[\bigg]{ \frac{ C_0 K }{1 - \Lambda^{-\holderexp}} (\diam{d}{S^{2}} )^{\holderexp} + 2n_{F} K }.
    \]
    Then we have $\Csplratio \leqslant \Csplratio'$ for each $\potential \in \holderspacesphere$ with $\holdernorm{\potential}{S^{2}} \leq K$, and the constant $\Csplratio'$ only depends on $F$, $\mathcal{C}$, $d$, $K$, and $\holderexp$. 

    Thus by \eqref{eq:temp:modulus of product of function and split operator}, we get that for $j \in \n_0$, $v \in \moduspace[][][S^2]$, and $\potential \in H$, 
    \begin{equation}    \label{eq:temp:upper bound for norm of second term}
        \normcontinuous[\bigg]{ \eigfun \int \! \widetilde{v} \, \normsplopt^{j} \bigl( \indicator{\splitsphere} \bigr) \,\mathrm{d}\spleigmea }{\splitsphere}
        \leqslant \normcontinuous{\eigfun}{\splitsphere} \normcontinuous[\Big]{\widetilde{v} \, \normsplopt^{j} \bigl( \indicator{\splitsphere} \bigr)}{\splitsphere}
        \leqslant \moduconst_1 \Csplratio'.
    \end{equation}
    By \eqref{eq:modulus for function under normed split Ruelle operator} in Proposition~\ref{prop:modulus for function under split ruelle operator} and \eqref{eq:temp:modulus of product of function and split operator}, we get some constant $\moduconst_2 > 0$ such that for each $j, \, k \in \n_0$, each $v \in \moduspace[][][S^2]$, and each $\potential \in H$,
    \begin{equation}    \label{eq:temp:upper bound for norm of first term}
        \normcontinuous[\Big]{\normsplopt^{k} \Bigl( \widetilde{v} \, \normsplopt^{j} \bigl( \indicator{\splitsphere} \bigr) \Bigr) }{\splitsphere} < \moduconst_2.
    \end{equation}
    Hence we can conclude from \eqref{eq:temp:upper bound for norm of second term}, \eqref{eq:temp:upper bound for norm of first term}, and \eqref{eq:temp:converge product function under operator} that
    \[
        \lim_{n \to +\infty} \frac{1}{n} \normcontinuous[\bigg]{ \sum\limits_{j=0}^{n-1} \normsplopt^{n - j}\Bigl( \widetilde{v} \, \normsplopt^{j} \bigl( \indicator{\splitsphere} \bigr) \Bigl) - \sum\limits_{j=0}^{n-1} \eigfun \int \! \widetilde{v} \, \normsplopt^{j} \bigl( \indicator{\splitsphere} \bigr) \,\mathrm{d}\spleigmea  }{\splitsphere} = 0,
    \]
    uniformly in $v \in \moduspace[][][S^2]$ and $\potential \in H$. Thus by \eqref{eq:temp:converge indicator under operator} and \eqref{eq:temp:bounds for norm of eigenfunction use in converge}, we have\[
        \lim_{n \to +\infty}  \normcontinuous[\Biggg]{ \frac{ \frac{1}{n} \sum\limits_{j=0}^{n-1} \normsplopt^{n - j}\Bigl( \widetilde{v} \, \normsplopt^{j} \bigl( \indicator{\splitsphere} \bigr) \Bigl)} { \normsplopt^{n}\bigl( \indicator{\splitsphere} \bigl) }  -  \frac{ \frac{1}{n} \sum\limits_{j=0}^{n-1} \eigfun \displaystyle\int \! \widetilde{v} \, \normsplopt^{j} \bigl( \indicator{\splitsphere} \bigr) \,\mathrm{d}\spleigmea }{\eigfun}  }{\splitsphere} = 0,
    \] 
    uniformly in $v \in \moduspace[][][S^2]$ and $\potential \in H$. Combining the above with \eqref{eq:temp:modulus of product of function and split operator}, \eqref{eq:temp:converge indicator under operator}, \eqref{eq:temp:bounds for norm of eigenfunction use in converge}, and the calculation at the beginning of the proof, we can conclude, therefore, that the left-hand side of \eqref{eq:converge of derivative for pressure of subsystem} is equal to 
    \[
        \begin{split}
            \lim_{n \to +\infty} \frac{1}{n} \sum\limits_{j = 0}^{n - 1} \int \! \widetilde{v} \, \normsplopt^{j} \bigl( \indicator{\splitsphere} \bigr) \,\mathrm{d}\spleigmea 
            &= \lim_{n \to +\infty} \frac{1}{n} \sum\limits_{j = 0}^{n - 1} \int \! \widetilde{v} \, \eigfun \,\mathrm{d}\spleigmea \\
            &= \int \! \widetilde{v} \,\mathrm{d}\splmea = \int \! v \,\mathrm{d}\equstate,
        \end{split}
    \]
    where $\equstate \in \probsphere$ is defined in Theorem~\ref{thm:existence of f invariant Gibbs measure}, and the convergence is uniform in $v \in \moduspace[][][S^2]$ and $\potential \in H$.
\end{proof}

We record the following well-known fact for the convenience of the reader.
\begin{lemma}    \label{lem:holder space dense in continuous space}
    Let $(X, d)$ be a compact metric space. 
    For each $\holderexp \in (0, 1]$, $\holderspace$ is a dense subset of $C(X)$ with respect to the uniform norm. 
    %In particular, $\holderspace$ is a dense subset of $C(X)$ in the weak topology.
\end{lemma}
\begin{proof}
    The lemma follows from the fact that the set of Lipschitz functions is dense in $C(X)$ with respect to the uniform norm (see for example, \cite[Theorem~6.8]{heinonen2001lectures}).
\end{proof}

\begin{theorem}    \label{thm:derivative of pressure subsystem}
    Let $f$, $\mathcal{C}$, $F$, $d$, $\potential$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive.
    Let $\potential, \, \gamma \in \holderspacesphere$ be real-valued \holder continuous function with an exponent $\holderexp \in (0, 1]$. 
    Then for each $t \in \real$, we have
    \[
        \frac{\mathrm{d}}{\mathrm{d}t} \pressure[\potential + t \gamma] = \int \! \gamma \,\mathrm{d}\equstate[\potential + t \gamma],
    \]
    where $\equstate[\potential + t \gamma] \in \probsphere$ is defined in Theorem~\ref{thm:existence of f invariant Gibbs measure}. 
\end{theorem}
\begin{proof}
    We will use the well-known fact from real analysis that if a sequence $\{g_{n}\}_{n \in \n}$ of real-valued differentiable functions defined on a finite interval in $\real$ converges pointwise to some function $g$ and the sequence of the corresponding derivatives $\bigl\{ \frac{\mathrm{d}g_{n}}{\mathrm{d}t} \bigr\}_{n \in \n}$ converges uniformly to some function $h$, then $g$ is differentiable and $\frac{dg}{\mathrm{d}t} = h$.

    By \eqref{eq:subsystem Variational Principle} in Theorem~\ref{thm:subsystem characterization of pressure}, Corollary~\ref{coro:well-define for split operator norm constant}, and \eqref{eq:iteration of split-partial ruelle operator} in Lemma~\ref{lem:iteration of split-partial ruelle operator}, for each $\colour \in \colours$, each $x \in X^0_{\colour}$, and each $\psi \in \holderspacesphere$, we have
    \begin{equation}    \label{eq:temp:characterization of pressure for subsystem}
        \begin{split}
            \pressure[\psi] &= \lim_{n \to +\infty} \frac{1}{n} \log \mathopen{}\bigl( \splopt[\psi]^{n}\bigl(\indicator{\splitsphere}\bigr)(x, \colour) \bigr) 
            = \lim_{n \to +\infty} \frac{1}{n} \log \sum\limits_{ X^n \in \ccFTile{n}{\colour}{} } \myexp[\big]{ S^{F}_{n} \psi( x_{X^{n}} ) },
        \end{split}
    \end{equation}
    where $x_{X^{n}} \define (F^{n}|_{X^{n}})^{-1}(x)$ for each $X^{n} \in \ccFTile{n}{\colour}{}$.

    Fix $\colour \in \colours$, $x \in X^0_{\colour}$, and $\ell \in (0, +\infty)$. 
    For $n \in \n$ and $t \in \real$, define\[
        P_n(t) \define \frac{1}{n} \log \sum_{ X^n \in \ccFTile{n}{\colour}{} } \myexp[\big]{ S^{F}_{n}(\phi + t \gamma)(x_{X^{n}}) },
    \]
    where $x_{X^{n}} \define (F^{n}|_{X^{n}})^{-1}(x)$ for each $X^{n} \in \ccFTile{n}{\colour}{}$.
    Observe that there exists a bounded subset $H$ of $\holderspacesphere$ such that $\phi + t \gamma \in H$ for each $t \in (-\ell, \ell)$. Then by Lemma~\ref{lem:converge of derivative for pressure of subsystem},\[
        \frac{\mathrm{d} P_{n}}{\mathrm{d}t}(t) = \frac{ \frac{1}{n} \sum\limits_{ X^n \in \ccFTile{n}{\colour}{} } \bigl(S_n^{F}\gamma( x_{X^{n}} )\bigr) \myexp[\big]{ S^{F}_{n} (\phi + t \gamma)(x_{X^{n}}) } }{ \sum\limits_{ X^n \in \ccFTile{n}{\colour}{} } \myexp[\big]{ S^{F}_{n} (\phi + t \gamma)(x_{X^{n}}) } }
    \]
    converges to $\int \! \gamma \,\mathrm{d}\equstate[\potential + t \gamma]$ as $n \to +\infty$, uniformly in $t \in (-\ell, \ell)$.

    On the other hand, by \eqref{eq:temp:characterization of pressure for subsystem}, for each $t \in (-\ell, \ell)$, we have\[
        \lim_{n \to +\infty}  P_{n}(t) = \pressure[\phi + t \gamma].
    \]
    Hence $\pressure[\phi + t \gamma]$ is differentiable with respect to $t$ on $(-\ell, \ell)$, and \[
        \frac{\mathrm{d}}{\mathrm{d}t} \pressure[\phi + t \gamma] = \lim_{n \to +\infty} \frac{\mathrm{d} P_{n}}{\mathrm{d}t}(t) = \int \! \gamma \,\mathrm{d}\equstate[\potential + t \gamma].
    \]
    Since $\ell \in (0, +\infty)$ is arbitrary, the proof is complete.
\end{proof}


Now we prove the uniqueness of the equilibrium states for subsystems. 
% We follow the conventions discussed in Remark~\ref{rem:invariant measure equivalent}. 

\begin{proof}[Proof of Theorem~\ref{thm:subsystem:uniqueness of equilibrium state}]
    The existence is proved in Theorem~\ref{thm:existence of equilibrium state for subsystem}. 
    
    We now prove the uniqueness.
    
    Denote $\limitset \define \limitset(F, \mathcal{C})$ and $\limitmap \define F|_{\limitset}$. 
    Recall that for each $\varphi \in C(S^2)$, $\fpressure[\varphi]$ is the topological pressure of $\limitmap \colon \limitset \mapping \limitset$ with respect to the potential $\varphi$. 

    Since $\potential \in \holderspacesphere$ for some $\holderexp \in (0, 1]$, it follows from Theorem~\ref{thm:subsystem characterization of pressure} and Theorem~\ref{thm:derivative of pressure subsystem} that the function \[
        t \mapsto \fpressure[\potential + t \gamma]
    \] 
    is differentiable at $0$ for each $\gamma \in \holderspacesphere$.
    Let \[
        W \define \bigl\{ \psi|_{\limitset} \in \holderspace[][][\limitset] \describe \psi \in \holderspacesphere \bigr\}.
    \] 
    By Lemma~\ref{lem:holder space dense in continuous space}, $W$ is a dense subset of $C(\limitset)$ with respect to the uniform norm.
    In particular, $W$ is a dense subset of $C(\limitset)$ in the weak topology.
    We note that the topological pressure function $\fpressure[\cdot] \colon C(\limitset) \mapping \real$ is convex continuous (see for example, \cite[Theorem~3.6.1 and Theorem~3.6.2]{przytycki2010conformal}). 
    Thus by Theorem~\ref{thm:tengent} with $V = C(\limitset)$, $x = \phi$, $U = W$, and $Q = \fpressure[\cdot]$, we get $\card[\big]{ \tangent{C(\limitset)}{\phi}{\fpressure[\cdot]} } = 1$.

    On the other hand, if $\mu \in \mathcal{M}(\limitset, \limitmap)$ is an equilibrium state for $\limitmap$ and $\potential$, then by \eqref{eq:def:measure-theoretic pressure} and \eqref{eq:Variational Principle for pressure},\[
        h_{\mu}(\limitmap) + \int \! \potential \,\mathrm{d}\mu = \fpressure[\potential],
    \]  
    and for each $\gamma \in C(\limitset)$,
    \[
        h_{\mu}(\limitmap) + \int \! (\potential + \gamma) \,\mathrm{d}\mu \leqslant \fpressure[\potential + \gamma].
    \]
    Thus $\int \! \gamma \,\mathrm{d}\mu \leqslant \fpressure[\potential + \gamma] - \fpressure[\potential]$. Then by \eqref{eq:def:tangent}, the continuous functional $\gamma \mapsto \int \! \gamma \,\mathrm{d}\mu$ on $C(\limitset)$ is in $\tangent{C(\limitset)}{\potential}{\fpressure[\cdot]}$. Since $\equstate$ defined in Theorem~\ref{thm:existence of f invariant Gibbs measure} is an equilibrium state for $\limitmap$ and $\potential$, and $\card[\big]{ \tangent{C(\limitset)}{\phi}{\fpressure[\cdot]} } = 1$, we get that each equilibrium state $\mu$ for $\limitmap$ and $\potential$ must satisfy $\int \! \gamma \,\mathrm{d}\mu = \int \! \gamma \,\mathrm{d}\equstate$ for $\gamma \in C(\limitset)$, i.e., $\mu = \equstate$.

    Finally, it follows from Theorem~\ref{thm:existence of equilibrium state for subsystem} that the map $\limitmap$ is forward quasi-invariant and non-singular with respect to $\equstate$.
\end{proof}

\begin{rmk}
    Let $f$, $\mathcal{C}$, $F$, $d$, $\potential$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}. 
    We assume in addition that $f(\mathcal{C}) \subseteq \mathcal{C}$ and $F \in \subsystem$ is strongly primitive.
    Since the entropy map $\mu \mapsto h_\mu(\limitmap)$ for $\limitmap \colon \limitset \mapping \limitset$ is \defn{affine} (see for example, \cite[Theorem~8.1]{walters1982introduction}), i.e., if $\juxtapose{\mu}{\nu} \in \invmea[\limitset][\limitmap]$ and $p \in [0, 1]$, then $h_{p\mu + (1 - p)\nu}(\limitmap) = p h_{\mu}(\limitmap) + (1 - p) h_{\nu}(\limitmap)$, so is the pressure map $\mu \mapsto P_{\mu}(\limitmap, \potential)$ for $\limitmap$ and $\potential$. 
    Thus, the uniqueness of the equilibrium state $\equstate$ and the Variational Principle~\eqref{eq:Variational Principle for pressure} imply that $\equstate$ is an extreme point of the convex set $\invmea[\limitset][\limitmap]$. 
    It follows from the fact (see for example, \cite[Theorem~2.2.8]{przytycki2010conformal}) that the extreme points of $\invmea[\limitset][\limitmap]$ are exactly the ergodic measures in $\invmea[\limitset][\limitmap]$ that $\equstate$ is ergodic. 
    However, we are going to prove a much stronger ergodic property of $\equstate$ in Section~\ref{sec:Ergodic Properties}.
\end{rmk}


Theorem~\ref{thm:subsystem:uniqueness of equilibrium state} implies in particular that there exists a unique equilibrium state $\mu_{\potential}$ for each expanding Thurston map $f \colon S^2 \mapping S^2$ together with a real-valued \holder continuous potential $\potential$.
\begin{corollary}    \label{coro:existence and uniqueness of equilibrium state for expanding Thurston map}
    Let $f$, $d$, $\potential$ satisfy the Assumptions in Section~\ref{sec:The Assumptions}.
    Then there exists a unique equilibrium state $\mu_{\potential}$ for the map $f$ and the potential $\potential$.
\end{corollary}
\begin{proof}
    By Lemma~\ref{lem:invariant_Jordan_curve} we can find a sufficiently high iterate $F \define f^n$ of $f$ for some $n \in \n$ that has an $F$-invariant Jordan curve $\mathcal{C} \subseteq S^2$ with $\post{F} = \post{f} \subseteq \mathcal{C}$. 
    Then $F$ is also an expanding Thurston map (Remark~\ref{rem:Expansion_is_independent}). In particular, $F$ is a strongly primitive subsystem of $F$ with respect to $\mathcal{C}$ (Remark~\ref{rem:expanding Thurston map is strongly primitive subsystem of itself}) and $\limitset(F, \mathcal{C}) = S^2$.

    Denote $\Phi \define S_{n}^{f} \potential$. By Theorem~\ref{thm:subsystem:uniqueness of equilibrium state} there exists a unique equilibrium state $\equstate[\Phi] \in \mathcal{M}(S^2, F)$ for the map $F$ and the potential $\Phi$. Note that $\equstate[\Phi]$ is $F$-invariant. Thus we have \[
        \mu \define \frac{1}{n} \sum_{i = 0}^{n - 1} f^{i}_{*} \equstate[\Phi] \in \mathcal{M}(S^2, f)
    \]
    and\[
        \int \! \potential \,\mathrm{d}\mu = \frac{1}{n} \int \sum_{i = 0}^{n - 1} \potential \,\mathrm{d}f_{*}^{i} \equstate[\Phi]
        = \frac{1}{n} \int \sum_{i = 0}^{n - 1} \potential \circ f^{i} \,\mathrm{d}\equstate[\Phi]
        = \frac{1}{n} \int \! \Phi \,\mathrm{d}\equstate[\Phi].
    \]
    By \eqref{eq:measure-theoretic entropy well-behaved under iteration} and \eqref{eq:measure-theoretic entropy is affine}, we have
    \begin{equation}    \label{eq:temp:coro:existence and uniqueness of equilibrium state for expanding Thurston map:equality for entropy}
        n h_{\mu}(f) = h_{\mu}(F) = \frac{1}{n} \sum_{i = 0}^{n - 1} h_{f_{*}^{i} \equstate[\Phi]}(F).
    \end{equation}
    We now show that $h_{f_{*}^{i} \equstate[\Phi]}(F) = h_{\equstate[\Phi]}(F)$ for each $i \in \zeroton[n - 1]$. 
    Indeed, the measure $f_{*} \equstate[\Phi]$ is $F$-invariant and the triple $(S^{2}, F, f_{*}\equstate[\Phi])$ is a factor of $(S^{2}, F, \equstate[\Phi])$ by the map $f$. %(see Subsection~\ref{sub:thermodynamic formalism} for the definition of factors) 
    It follows that $h_{f_{*}\equstate[\Phi]}(F) \leqslant h_{\equstate[\Phi]}(F)$ (see Subsection~\ref{sub:thermodynamic formalism}). 
    Iterating this and noting that $f_{*}^{n} \equstate[\Phi] = (F)_{*}\equstate[\Phi] = \equstate[\Phi]$ by $F$-invariance of $\equstate[\Phi]$, we obtain\[
        h_{\equstate[\Phi]}(F) = h_{f_{*}^{n} \equstate[\Phi]}(F) 
        \leqslant h_{f_{*}^{n - 1} \equstate[\Phi]}(F) \leqslant \cdots 
        \leqslant h_{f_{*} \equstate[\Phi]}(F) \leqslant h_{\equstate[\Phi]}(F).
    \]
    Hence $h_{f_{*}^{i} \equstate[\Phi]}(f^n) = h_{\equstate[\Phi]}(F)$ for each $i \in \zeroton[n - 1]$. Combining this with \eqref{eq:temp:coro:existence and uniqueness of equilibrium state for expanding Thurston map:equality for entropy}, we obtain $n h_{\mu}(f) = h_{\equstate[\Phi]}(F)$.
    Noting that $P(F, \Phi) = n P(f, \potential)$ (recall \eqref{eq:def:topological pressure}), we get\[
         h_{\mu}(f) + \int \! \phi \,\mathrm{d}\mu
        = \frac{1}{n} \biggl( h_{\equstate[\Phi]}(F) + \int \! \Phi \,\mathrm{d}\equstate[\Phi] \biggr)
        = \frac{1}{n} P(F, \Phi) = P(f, \potential).
    \]
    Thus $\mu$ is an equilibrium state for the map $f$ and the potential $\potential$.

    Now we prove the uniqueness. Suppose $\nu$ is an equilibrium state for the map $f$ and the potential $\potential$. By similar arguments as above one sees that $\nu$ is an equilibrium state for the map $F$ and the potential $\Phi$. Then it follows from the uniqueness part of Theorem~\ref{thm:subsystem:uniqueness of equilibrium state} that $\nu = \equstate[\Phi]$.
\end{proof}

==> section/Tile_graph.tex <==
% !TEX root = ../main.tex

\section{Tile graphs}
\label{sec:Tile graphs}

In this section we study the properties of tile graphs of subsystems of expanding Thurston maps.

show that the entropy map of an expanding Thurston map with at least one periodic critical point is not upper semi-continuous.

